Type Safe Redis Queries: A Case Study of Type-Level Programming in Haskell

Redis is an in-memory data structure store, often used as a database, with a Haskell interface Hedis. Redis is dynamically typed --- a key can be discarded and re-associated to a value of a different type, and a command, when fetching a value of a type it does not expect, signals a runtime error. We develop a domain-specific language that, by exploiting Haskell type-level programming techniques including indexed monad, type-level literals and closed type families, keeps track of types of values in the database and statically guarantees that type errors cannot happen for a class of Redis programs.

==> Makefile <==
#-----------------------------------------------------------------------------
# Programs
#-----------------------------------------------------------------------------
LHS2TEX     := lhs2TeX
PDFLATEX    := pdflatex
LATEX       := latex
BIBTEX      := bibtex
GHCI        := ghci


#-----------------------------------------------------------------------------
# Directories and source files
#-----------------------------------------------------------------------------
MAIN        := main-tyde
MAINTECH    := 
SRCDIR      := sections
LHSFILES    := $(wildcard $(SRCDIR)/*.lhs)
TEXFILES    := $(wildcard $(SRCDIR)/*.tex)

#-----------------------------------------------------------------------------
# Flags
#-----------------------------------------------------------------------------
GHCFLAGS      := -Wall -O
LHS2TEX_FLAGS := --poly
SPELL         := ispell -d british -t -l -p

all: $(MAIN).pdf
supplement: $(SRCDIR)/Supplement.pdf

# $(MAINTECH).pdf

#-----------------------------------------------------------------------------
# Pattern rules
#-----------------------------------------------------------------------------

$(MAINTECH).pdf: $(MAINTECH).tex lhs $(TEXFILES) force
	$(PDFLATEX) $<
	if grep -s '^LaTeX Warning: Citation' $(<:.tex=.log); \
	then $(BIBTEX) $(<:.tex=); $(PDFLATEX) $(<); \
	fi
	while grep -s "Warning.*Rerun" $(<:.tex=.log); \
	  do $(PDFLATEX) $<; done;

%.tex : %.lhs force
	[ $(<) ] && ($(LHS2TEX) $(LHS2TEX_FLAGS) $< > $@ || rm -f $@)

#-----------------------------------------------------------------------------
# Rules
#-----------------------------------------------------------------------------

$(MAIN).pdf: $(MAIN).tex lhs $(TEXFILES) force
	$(PDFLATEX) $(<)
	if grep -s '^LaTeX Warning: Citation' $(<:.tex=.log); \
	then $(BIBTEX) $(<:.tex=); $(LATEX) $(<); \
	fi
	while grep -s "Warning.*Rerun" $(<:.tex=.log); \
	  do $(PDFLATEX) $<; done;

$(SRCDIR)/Supplement.pdf: $(SRCDIR)/Supplement.tex lhs $(TEXFILES)
	$(PDFLATEX) $(<)
	if grep -s '^LaTeX Warning: Citation' $(<:.tex=.log); \
	then $(BIBTEX) $(<:.tex=); $(LATEX) $(<); \
	fi
	while grep -s "Warning.*Rerun" $(<:.tex=.log); \
	  do $(PDFLATEX) $<; done;

lhs: $(LHSFILES:.lhs=.tex)

ghci: $(file).lhs
	ghci $(file).lhs

spell: $(file).tex
	egrep -v '$\%' $(file).tex | $(spell) $(file).spell | sort | uniq

force:

clean:
	rm -vf $(LHSFILES:.lhs=.tex)
	rm -vf *.pdf
	rm -vf *.dvi
	rm -vf *.aux *.log *.bbl *.blg *.ptb
	rm -rfv auto _region_.tex

.PHONY: ghci spell force clean


==> Preamble.tex <==
%%include lhs2TeX.fmt
%% ODER: format ==         = "\mathrel{==}"
%% ODER: format /=         = "\neq "
%
%
\makeatletter
\@ifundefined{lhs2tex.lhs2tex.sty.read}%
  {\@namedef{lhs2tex.lhs2tex.sty.read}{}%
   \newcommand\SkipToFmtEnd{}%
   \newcommand\EndFmtInput{}%
   \long\def\SkipToFmtEnd#1\EndFmtInput{}%
  }\SkipToFmtEnd

\newcommand\ReadOnlyOnce[1]{\@ifundefined{#1}{\@namedef{#1}{}}\SkipToFmtEnd}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{stmaryrd}
\DeclareFontFamily{OT1}{cmtex}{}
\DeclareFontShape{OT1}{cmtex}{m}{n}
  {<5><6><7><8>cmtex8
   <9>cmtex9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmtex10}{}
\DeclareFontShape{OT1}{cmtex}{m}{it}
  {<-> ssub * cmtt/m/it}{}
\newcommand{\texfamily}{\fontfamily{cmtex}\selectfont}
\DeclareFontShape{OT1}{cmtt}{bx}{n}
  {<5><6><7><8>cmtt8
   <9>cmbtt9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmbtt10}{}
\DeclareFontShape{OT1}{cmtex}{bx}{n}
  {<-> ssub * cmtt/bx/n}{}
\newcommand{\tex}[1]{\text{\texfamily#1}}	% NEU

\newcommand{\Sp}{\hskip.33334em\relax}


\newcommand{\Conid}[1]{\mathit{#1}}
\newcommand{\Varid}[1]{\mathit{#1}}
\newcommand{\anonymous}{\kern0.06em \vbox{\hrule\@width.5em}}
\newcommand{\plus}{\mathbin{+\!\!\!+}}
\newcommand{\bind}{\mathbin{>\!\!\!>\mkern-6.7mu=}}
\newcommand{\rbind}{\mathbin{=\mkern-6.7mu<\!\!\!<}}% suggested by Neil Mitchell
\newcommand{\sequ}{\mathbin{>\!\!\!>}}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\usepackage{polytable}

%mathindent has to be defined
\@ifundefined{mathindent}%
  {\newdimen\mathindent\mathindent\leftmargini}%
  {}%

\def\resethooks{%
  \global\let\SaveRestoreHook\empty
  \global\let\ColumnHook\empty}
\newcommand*{\savecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\savecolumns[#1]}}
\newcommand*{\restorecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\restorecolumns[#1]}}
\newcommand*{\aligncolumn}[2]%
  {\g@addto@macro\ColumnHook{\column{#1}{#2}}}

\resethooks

\newcommand{\onelinecommentchars}{\quad-{}- }
\newcommand{\commentbeginchars}{\enskip\{-}
\newcommand{\commentendchars}{-\}\enskip}

\newcommand{\visiblecomments}{%
  \let\onelinecomment=\onelinecommentchars
  \let\commentbegin=\commentbeginchars
  \let\commentend=\commentendchars}

\newcommand{\invisiblecomments}{%
  \let\onelinecomment=\empty
  \let\commentbegin=\empty
  \let\commentend=\empty}

\visiblecomments

\newlength{\blanklineskip}
\setlength{\blanklineskip}{0.66084ex}

\newcommand{\hsindent}[1]{\quad}% default is fixed indentation
\let\hspre\empty
\let\hspost\empty
\newcommand{\NB}{\textbf{NB}}
\newcommand{\Todo}[1]{$\langle$\textbf{To do:}~#1$\rangle$}

\EndFmtInput
\makeatother
%
%
%
%
%
%
% This package provides two environments suitable to take the place
% of hscode, called "plainhscode" and "arrayhscode". 
%
% The plain environment surrounds each code block by vertical space,
% and it uses \abovedisplayskip and \belowdisplayskip to get spacing
% similar to formulas. Note that if these dimensions are changed,
% the spacing around displayed math formulas changes as well.
% All code is indented using \leftskip.
%
% Changed 19.08.2004 to reflect changes in colorcode. Should work with
% CodeGroup.sty.
%
\ReadOnlyOnce{polycode.fmt}%
\makeatletter

\newcommand{\hsnewpar}[1]%
  {{\parskip=0pt\parindent=0pt\par\vskip #1\noindent}}

% can be used, for instance, to redefine the code size, by setting the
% command to \small or something alike
\newcommand{\hscodestyle}{}

% The command \sethscode can be used to switch the code formatting
% behaviour by mapping the hscode environment in the subst directive
% to a new LaTeX environment.

\newcommand{\sethscode}[1]%
  {\expandafter\let\expandafter\hscode\csname #1\endcsname
   \expandafter\let\expandafter\endhscode\csname end#1\endcsname}

% "compatibility" mode restores the non-polycode.fmt layout.

\newenvironment{compathscode}%
  {\par\noindent
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \par\noindent
   \ignorespacesafterend}

\newcommand{\compaths}{\sethscode{compathscode}}

% "plain" mode is the proposed default.

\newenvironment{plainhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

% Here, we make plainhscode the default environment.

\newcommand{\plainhs}{\sethscode{plainhscode}}
\plainhs

% The arrayhscode is like plain, but makes use of polytable's
% parray environment which disallows page breaks in code blocks.

\newenvironment{arrayhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\parray}%
  {\endparray\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

\newcommand{\arrayhs}{\sethscode{arrayhscode}}

% The mathhscode environment also makes use of polytable's parray 
% environment. It is supposed to be used only inside math mode 
% (I used it to typeset the type rules in my thesis).

\newenvironment{mathhscode}%
  {\parray}{\endparray}

\newcommand{\mathhs}{\sethscode{mathhscode}}

% texths is similar to mathhs, but works in text mode.

\newenvironment{texthscode}%
  {\(\parray}{\endparray\)}

\newcommand{\texths}{\sethscode{texthscode}}

% The framed environment places code in a framed box.

\def\codeframewidth{\arrayrulewidth}
\RequirePackage{calc}

\newenvironment{framedhscode}%
  {\parskip=\abovedisplayskip\par\noindent
   \hscodestyle
   \arrayrulewidth=\codeframewidth
   \tabular{@{}|p{\linewidth-2\arraycolsep-2\arrayrulewidth-2pt}|@{}}%
   \hline\framedhslinecorrect\\{-1.5ex}%
   \let\endoflinesave=\\
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \framedhslinecorrect\endoflinesave{.5ex}\hline
   \endtabular
   \parskip=\belowdisplayskip\par\noindent
   \ignorespacesafterend}

\newcommand{\framedhslinecorrect}[2]%
  {#1[#2]}

\newcommand{\framedhs}{\sethscode{framedhscode}}

% The inlinehscode environment is an experimental environment
% that can be used to typeset displayed code inline.

\newenvironment{inlinehscode}%
  {\(\def\column##1##2{}%
   \let\>\undefined\let\<\undefined\let\\\undefined
   \newcommand\>[1][]{}\newcommand\<[1][]{}\newcommand\\[1][]{}%
   \def\fromto##1##2##3{##3}%
   \def\nextline{}}{\) }%

\newcommand{\inlinehs}{\sethscode{inlinehscode}}

% The joincode environment is a separate environment that
% can be used to surround and thereby connect multiple code
% blocks.

\newenvironment{joincode}%
  {\let\orighscode=\hscode
   \let\origendhscode=\endhscode
   \def\endhscode{\def\hscode{\endgroup\def\@currenvir{hscode}\\}\begingroup}
   %\let\SaveRestoreHook=\empty
   %\let\ColumnHook=\empty
   %\let\resethooks=\empty
   \orighscode\def\hscode{\endgroup\def\@currenvir{hscode}}}%
  {\origendhscode
   \global\let\hscode=\orighscode
   \global\let\endhscode=\origendhscode}%

\makeatother
\EndFmtInput
%


==> sections/Embedding-orig.tex <==
%% ODER: format ==         = "\mathrel{==}"
%% ODER: format /=         = "\neq "
%
%
\makeatletter
\@ifundefined{lhs2tex.lhs2tex.sty.read}%
  {\@namedef{lhs2tex.lhs2tex.sty.read}{}%
   \newcommand\SkipToFmtEnd{}%
   \newcommand\EndFmtInput{}%
   \long\def\SkipToFmtEnd#1\EndFmtInput{}%
  }\SkipToFmtEnd

\newcommand\ReadOnlyOnce[1]{\@ifundefined{#1}{\@namedef{#1}{}}\SkipToFmtEnd}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{stmaryrd}
\DeclareFontFamily{OT1}{cmtex}{}
\DeclareFontShape{OT1}{cmtex}{m}{n}
  {<5><6><7><8>cmtex8
   <9>cmtex9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmtex10}{}
\DeclareFontShape{OT1}{cmtex}{m}{it}
  {<-> ssub * cmtt/m/it}{}
\newcommand{\texfamily}{\fontfamily{cmtex}\selectfont}
\DeclareFontShape{OT1}{cmtt}{bx}{n}
  {<5><6><7><8>cmtt8
   <9>cmbtt9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmbtt10}{}
\DeclareFontShape{OT1}{cmtex}{bx}{n}
  {<-> ssub * cmtt/bx/n}{}
\newcommand{\tex}[1]{\text{\texfamily#1}}	% NEU

\newcommand{\Sp}{\hskip.33334em\relax}


\newcommand{\Conid}[1]{\mathit{#1}}
\newcommand{\Varid}[1]{\mathit{#1}}
\newcommand{\anonymous}{\kern0.06em \vbox{\hrule\@width.5em}}
\newcommand{\plus}{\mathbin{+\!\!\!+}}
\newcommand{\bind}{\mathbin{>\!\!\!>\mkern-6.7mu=}}
\newcommand{\rbind}{\mathbin{=\mkern-6.7mu<\!\!\!<}}% suggested by Neil Mitchell
\newcommand{\sequ}{\mathbin{>\!\!\!>}}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\usepackage{polytable}

%mathindent has to be defined
\@ifundefined{mathindent}%
  {\newdimen\mathindent\mathindent\leftmargini}%
  {}%

\def\resethooks{%
  \global\let\SaveRestoreHook\empty
  \global\let\ColumnHook\empty}
\newcommand*{\savecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\savecolumns[#1]}}
\newcommand*{\restorecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\restorecolumns[#1]}}
\newcommand*{\aligncolumn}[2]%
  {\g@addto@macro\ColumnHook{\column{#1}{#2}}}

\resethooks

\newcommand{\onelinecommentchars}{\quad-{}- }
\newcommand{\commentbeginchars}{\enskip\{-}
\newcommand{\commentendchars}{-\}\enskip}

\newcommand{\visiblecomments}{%
  \let\onelinecomment=\onelinecommentchars
  \let\commentbegin=\commentbeginchars
  \let\commentend=\commentendchars}

\newcommand{\invisiblecomments}{%
  \let\onelinecomment=\empty
  \let\commentbegin=\empty
  \let\commentend=\empty}

\visiblecomments

\newlength{\blanklineskip}
\setlength{\blanklineskip}{0.66084ex}

\newcommand{\hsindent}[1]{\quad}% default is fixed indentation
\let\hspre\empty
\let\hspost\empty
\newcommand{\NB}{\textbf{NB}}
\newcommand{\Todo}[1]{$\langle$\textbf{To do:}~#1$\rangle$}

\EndFmtInput
\makeatother
%
%
%
%
%
%
% This package provides two environments suitable to take the place
% of hscode, called "plainhscode" and "arrayhscode". 
%
% The plain environment surrounds each code block by vertical space,
% and it uses \abovedisplayskip and \belowdisplayskip to get spacing
% similar to formulas. Note that if these dimensions are changed,
% the spacing around displayed math formulas changes as well.
% All code is indented using \leftskip.
%
% Changed 19.08.2004 to reflect changes in colorcode. Should work with
% CodeGroup.sty.
%
\ReadOnlyOnce{polycode.fmt}%
\makeatletter

\newcommand{\hsnewpar}[1]%
  {{\parskip=0pt\parindent=0pt\par\vskip #1\noindent}}

% can be used, for instance, to redefine the code size, by setting the
% command to \small or something alike
\newcommand{\hscodestyle}{}

% The command \sethscode can be used to switch the code formatting
% behaviour by mapping the hscode environment in the subst directive
% to a new LaTeX environment.

\newcommand{\sethscode}[1]%
  {\expandafter\let\expandafter\hscode\csname #1\endcsname
   \expandafter\let\expandafter\endhscode\csname end#1\endcsname}

% "compatibility" mode restores the non-polycode.fmt layout.

\newenvironment{compathscode}%
  {\par\noindent
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \let\hspre\(\let\hspost\)%
   \pboxed}%
  {\endpboxed\)%
   \par\noindent
   \ignorespacesafterend}

\newcommand{\compaths}{\sethscode{compathscode}}

% "plain" mode is the proposed default.
% It should now work with \centering.
% This required some changes. The old version
% is still available for reference as oldplainhscode.

\newenvironment{plainhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\hspre\(\let\hspost\)%
   \pboxed}%
  {\endpboxed%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

\newenvironment{oldplainhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

% Here, we make plainhscode the default environment.

\newcommand{\plainhs}{\sethscode{plainhscode}}
\newcommand{\oldplainhs}{\sethscode{oldplainhscode}}
\plainhs

% The arrayhscode is like plain, but makes use of polytable's
% parray environment which disallows page breaks in code blocks.

\newenvironment{arrayhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\parray}%
  {\endparray\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

\newcommand{\arrayhs}{\sethscode{arrayhscode}}

% The mathhscode environment also makes use of polytable's parray 
% environment. It is supposed to be used only inside math mode 
% (I used it to typeset the type rules in my thesis).

\newenvironment{mathhscode}%
  {\parray}{\endparray}

\newcommand{\mathhs}{\sethscode{mathhscode}}

% texths is similar to mathhs, but works in text mode.

\newenvironment{texthscode}%
  {\(\parray}{\endparray\)}

\newcommand{\texths}{\sethscode{texthscode}}

% The framed environment places code in a framed box.

\def\codeframewidth{\arrayrulewidth}
\RequirePackage{calc}

\newenvironment{framedhscode}%
  {\parskip=\abovedisplayskip\par\noindent
   \hscodestyle
   \arrayrulewidth=\codeframewidth
   \tabular{@{}|p{\linewidth-2\arraycolsep-2\arrayrulewidth-2pt}|@{}}%
   \hline\framedhslinecorrect\\{-1.5ex}%
   \let\endoflinesave=\\
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \framedhslinecorrect\endoflinesave{.5ex}\hline
   \endtabular
   \parskip=\belowdisplayskip\par\noindent
   \ignorespacesafterend}

\newcommand{\framedhslinecorrect}[2]%
  {#1[#2]}

\newcommand{\framedhs}{\sethscode{framedhscode}}

% The inlinehscode environment is an experimental environment
% that can be used to typeset displayed code inline.

\newenvironment{inlinehscode}%
  {\(\def\column##1##2{}%
   \let\>\undefined\let\<\undefined\let\\\undefined
   \newcommand\>[1][]{}\newcommand\<[1][]{}\newcommand\\[1][]{}%
   \def\fromto##1##2##3{##3}%
   \def\nextline{}}{\) }%

\newcommand{\inlinehs}{\sethscode{inlinehscode}}

% The joincode environment is a separate environment that
% can be used to surround and thereby connect multiple code
% blocks.

\newenvironment{joincode}%
  {\let\orighscode=\hscode
   \let\origendhscode=\endhscode
   \def\endhscode{\def\hscode{\endgroup\def\@currenvir{hscode}\\}\begingroup}
   %\let\SaveRestoreHook=\empty
   %\let\ColumnHook=\empty
   %\let\resethooks=\empty
   \orighscode\def\hscode{\endgroup\def\@currenvir{hscode}}}%
  {\origendhscode
   \global\let\hscode=\orighscode
   \global\let\endhscode=\origendhscode}%

\makeatother
\EndFmtInput
%

\ReadOnlyOnce{Formatting.fmt}%
\makeatletter

\let\Varid\mathit
\let\Conid\mathsf

\def\commentbegin{\quad\{\ }
\def\commentend{\}}

\newcommand{\ty}[1]{\Conid{#1}}
\newcommand{\con}[1]{\Conid{#1}}
\newcommand{\id}[1]{\Varid{#1}}
\newcommand{\cl}[1]{\Varid{#1}}
\newcommand{\opsym}[1]{\mathrel{#1}}

\newcommand\Keyword[1]{\textbf{\textsf{#1}}}
\newcommand\Hide{\mathbin{\downarrow}}
\newcommand\Reveal{\mathbin{\uparrow}}


%% Paper-specific keywords


\makeatother
\EndFmtInput

\section{Embedding \Hedis{} Commands}
\label{sec:embedding-commands}

Having the indexed monads and type-level dictionaries, in this section we
present our embedding of \Hedis{} commands into \Edis{}, while introducing
necessary concepts when they are used.

\subsection{Proxies and Singleton Types}
\label{sec:proxy-key}

The \Hedis{} function \ensuremath{\Varid{del}\mathbin{::}[\mskip1.5mu \Conid{ByteString}\mskip1.5mu]\to \Conid{Redis}\;(\Conid{R} \uplus \Conid{Integer})} takes a list of keys (encoded to \ensuremath{\Conid{ByteString}}) and removes the entries having those
keys in the database. For some reason to be explained later, we consider an \Edis{}
counterpart that takes only one key. A first attempt may lead to something like
the following:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{del}\mathbin{::}\Conid{String}\to \Conid{Edis}\;\Varid{xs}\;(\Conid{Del}\;\Varid{xs}~\mathbin{?})\;(\Conid{R} \uplus \Conid{Integer}){}\<[E]%
\\
\>[B]{}\Varid{del}\;\Varid{key}\mathrel{=}\Conid{Edis}\;(\Varid{\Conid{Hedis}.del}\;[\mskip1.5mu \Varid{encode}\;\Varid{key}\mskip1.5mu])~~,{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
where the function \ensuremath{\Varid{encode}} converts \ensuremath{\Conid{String}} to \ensuremath{\Conid{ByteString}}. At term-level,
our \ensuremath{\Varid{del}} merely calls \ensuremath{\Varid{\Conid{Hedis}.del}}. At type-level, if the status of the database
before \ensuremath{\Varid{del}} is called meets the constraint represented by the dictionary
\ensuremath{\Varid{xs}}, the status afterwards should meet the constraint \ensuremath{\Conid{Del}\;\Varid{xs}~\mathbin{?}}. The question, however, is what to fill in place of the question mark. It cannot be
\ensuremath{\Conid{Del}\;\Varid{xs}\;\Varid{key}}, since \ensuremath{\Varid{key}} is a runtime value and not a type. How do we smuggle
a runtime value to type-level?

In a language with phase distinction like Haskell, it is certainly impossible
to pass the value of \ensuremath{\Varid{key}} to the type checker if it truly is a runtime value,
for example, a string read from the user. If the value of \ensuremath{\Varid{key}} can be
determined statically, however, {\em singleton types} can be used to represent a
type as a value, thus build a connection between the two realms.

A singleton type is a type that has only one term. When the term is built, it
carries a type that can be inspected by the type checker. The term can be
thought of as a representative of its type at the realm of runtime values. For
our purpose, we will use the following type \ensuremath{\Conid{Proxy}}:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\mathbf{data}\;\Conid{Proxy}\;\Varid{t}\mathrel{=}\Conid{Proxy}~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
For every type \ensuremath{\Varid{t}}, \ensuremath{\Conid{Proxy}\;\Varid{t}} is a type that has only one term: \ensuremath{\Conid{Proxy}}.%
\footnote{While giving the same name to both the type and the term can be very
confusing, it is unfortunately a common practice in the Haskell community.}
To call \ensuremath{\Varid{del}}, instead of passing a key as a \ensuremath{\Conid{String}} value, we give it a proxy
with a specified type:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{del}\;(\Conid{Proxy}\mathbin{::}\Conid{Proxy}\;\text{\tt \char34 A\char34})~~,{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
where \ensuremath{\text{\tt \char34 A\char34}} is not a value, but a string lifted to a type (of kind \ensuremath{\Conid{Symbol}}).
Now that the type checker has access to the key, the type of \ensuremath{\Varid{del}} can be
\ensuremath{\Conid{Proxy}\;\Varid{k}\to \Conid{Edis}\;\Varid{xs}\;(\Conid{Del}\;\Varid{xs}\;\Varid{k})\;(\Conid{R} \uplus \Conid{Integer})}.

The next problem is that, \ensuremath{\Varid{del}}, at term level, gets only a value constructor
\ensuremath{\Conid{Proxy}} without further information, while it needs to pass a \ensuremath{\Conid{ByteString}} key
to \ensuremath{\Varid{\Conid{Hedis}.del}}. Every concrete string literal lifted to a type, for example,
\ensuremath{\text{\tt \char34 A\char34}}, belongs to a type class \ensuremath{\Conid{KnownSymbol}}. For all type \ensuremath{\Varid{k}} in \ensuremath{\Conid{KnownSymbol}},
the function \ensuremath{\Varid{symbolVal}}:\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{3}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[3]{}\Varid{symbolVal}\mathbin{::}\Conid{KnownSymbol}\;\Varid{k}\Rightarrow \Varid{proxy}\;\Varid{k}\to \Conid{String}~~,{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
retrieves the string associated with a type-level literal that is known at
compile time. In summary, \ensuremath{\Varid{del}} can be implemented as:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{6}{@{}>{\hspre}l<{\hspost}@{}}%
\column{45}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{del}{}\<[6]%
\>[6]{}\mathbin{::}\Conid{KnownSymbol}\;\Varid{k}{}\<[E]%
\\
\>[6]{}\Rightarrow \Conid{Proxy}\;\Varid{k}\to \Conid{Edis}\;\Varid{xs}\;(\Conid{Del}\;\Varid{xs}\;\Varid{k})\;(\Conid{R} \uplus \Conid{Integer}){}\<[E]%
\\
\>[B]{}\Varid{del}\;\Varid{key}\mathrel{=}\Conid{Edis}\;(\Varid{\Conid{Hedis}.del}\;[\mskip1.5mu \Varid{encodeKey}\;\Varid{key}\mskip1.5mu]){}\<[45]%
\>[45]{}~~,{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
where \ensuremath{\Varid{encodeKey}\mathrel{=}\Varid{encode}\mathbin{\cdot}\Varid{symbolVal}}.

A final note: the function \ensuremath{\Varid{encode}}, from the Haskell library {\sc cereal},
helps to convert certain datatypes that are {\em serializable} into \ensuremath{\Conid{ByteString}}.
The function and its dual \ensuremath{\Varid{decode}} will be used more later.
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{9}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{encode}{}\<[9]%
\>[9]{}\mathbin{::}\Conid{Serialize}\;\Varid{a}\Rightarrow \Varid{a}\to \Conid{ByteString}~~,{}\<[E]%
\\
\>[B]{}\Varid{decode}{}\<[9]%
\>[9]{}\mathbin{::}\Conid{Serialize}\;\Varid{a}\Rightarrow \Conid{ByteString}\to \Conid{Either}\;\Conid{String}\;\Varid{a}~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks

\subsection{Automatic Serialization}
\label{sec:polymorphic-redis}

As mentioned before, while \Redis{} provide a number of container types
including lists, sets, and hash, etc., the primitive type is string. \Hedis{}
programmers manually convert data of other types to strings before saving them
into the data store. In \Edis{}, we wish to save some of the effort for the
programmers, as well as keeping a careful record of the intended types of the
strings in the data store.

To keep track of intended types of strings in the data store, we define the
following types (that have no terms):
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{16}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\mathbf{data}\;\Conid{StringOf}{}\<[16]%
\>[16]{}\mathbin{::}\mathbin{*}\to \mathbin{*}~~,{}\<[E]%
\\
\>[B]{}\mathbf{data}\;\Conid{ListOf}{}\<[16]%
\>[16]{}\mathbin{::}\mathbin{*}\to \mathbin{*}~~,{}\<[E]%
\\
\>[B]{}\mathbf{data}\;\Conid{SetOf}{}\<[16]%
\>[16]{}\mathbin{::}\mathbin{*}\to \mathbin{*}~~...{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
If a key is associated with, for example, \ensuremath{\Conid{StringOf}\;\Conid{Int}} in our dictionary, we
mean that its value in the data store was serialized from an \ensuremath{\Conid{Int}} and should be
used as an \ensuremath{\Conid{Int}}. Types \ensuremath{\Conid{ListOf}\;\Varid{a}} and \ensuremath{\Conid{SetOf}\;\Varid{a}}, respectively, denotes that the
value is a list or a set of type \ensuremath{\Varid{a}}.

While the \ensuremath{\Varid{set}} command in \Hedis{} always writes a string to the data store,
the corresponding \ensuremath{\Varid{set}} in \Redis{} applies to any serializable type (those
in the class \ensuremath{\Conid{Serialize}}), and performs the encoding for the user:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{6}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{set}{}\<[6]%
\>[6]{}\mathbin{::}(\Conid{KnownSymbol}\;\Varid{k},\Conid{Serialize}\;\Varid{a}){}\<[E]%
\\
\>[6]{}\Rightarrow \Conid{Proxy}\;\Varid{k}\to \Varid{a}\to \Conid{Edis}\;\Varid{xs}\;(\Conid{Set}\;\Varid{xs}\;\Varid{k}\;(\Conid{StringOf}\;\Varid{a}))\;(\Conid{Either}\;\Conid{Reply}\;\Conid{Status}){}\<[E]%
\\
\>[B]{}\Varid{set}\;\Varid{key}\;\Varid{val}\mathrel{=}\Conid{Edis}\;(\Varid{\Conid{Hedis}.set}\;(\Varid{encodeKey}\;\Varid{key})\;(\Varid{encode}\;\Varid{val}))~~,{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
For example, executing \ensuremath{\Varid{set}\;(\Conid{Proxy}\mathbin{::}\Conid{Proxy}\;\text{\tt \char34 A\char34})\;\Conid{True}} updates the dictionary
with an entry \ensuremath{\mbox{\textquotesingle}(\text{\tt \char34 A\char34},\Conid{StringOf}\;\Conid{Bool})}. If \ensuremath{\text{\tt \char34 A\char34}} is not in the dictionary,
this entry is added; otherwise the old type of \ensuremath{\text{\tt \char34 A\char34}} is updated to
\ensuremath{\Conid{StringOf}\;\Conid{Bool}}.

\Redis{} command \texttt{INCR} reads the (string) value of the given key, parses
it as an integer, and increments it by one, before storing it back. The command
\texttt{INCRBYFLOAT} increments the floating point value of a key by a given
amount. They are defined in \Edis{} below:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{7}{@{}>{\hspre}l<{\hspost}@{}}%
\column{14}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{incr}{}\<[7]%
\>[7]{}\mathbin{::}(\Conid{KnownSymbol}\;\Varid{k},\Conid{Get}\;\Varid{xs}\;\Varid{k}\mathrel{\sim}\Conid{StringOf}\;\Conid{Integer}){}\<[E]%
\\
\>[7]{}\Rightarrow \Conid{Proxy}\;\Varid{k}\to \Conid{Edis}\;\Varid{xs}\;\Varid{xs}\;(\Conid{R} \uplus \Conid{Integer}){}\<[E]%
\\
\>[B]{}\Varid{incr}\;\Varid{key}\mathrel{=}\Conid{Edis}\;(\Varid{\Conid{Hedis}.incr}\;(\Varid{encodeKey}\;\Varid{key}))~~,{}\<[E]%
\\[\blanklineskip]%
\>[B]{}\Varid{incrbyfloat}{}\<[14]%
\>[14]{}\mathbin{::}(\Conid{KnownSymbol}\;\Varid{k},\Conid{Get}\;\Varid{xs}\;\Varid{k}\mathrel{\sim}\Conid{StringOf}\;\Conid{Double}){}\<[E]%
\\
\>[14]{}\Rightarrow \Conid{Proxy}\;\Varid{k}\to \Conid{Double}\to \Conid{Edis}\;\Varid{xs}\;\Varid{xs}\;(\Conid{R} \uplus \Conid{Double}){}\<[E]%
\\
\>[B]{}\Varid{incrbyfloat}\;\Varid{key}\;\Varid{eps}\mathrel{=}\Conid{Edis}\;(\Varid{\Conid{Hedis}.incrbyfloat}\;(\Varid{encodeKey}\;\Varid{key})\;\Varid{eps})~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
Notice the use of (\ensuremath{\mathrel{\sim}}), \emph{equality constraints}~\cite{typeeq}, to enforce
that the intended type of the value of \ensuremath{\Varid{k}} must respectively be \ensuremath{\Conid{Integer}} and
\ensuremath{\Conid{Double}}. The function \ensuremath{\Varid{incr}} is only allowed to be called in a context where
the type checker is able to reduce \ensuremath{\Conid{Get}\;\Varid{xs}\;\Varid{k}} to \ensuremath{\Conid{StringOf}\;\Conid{Integer}} ---
recall that when \ensuremath{\Varid{k}} is not in \ensuremath{\Varid{xs}}, \ensuremath{\Conid{Get}\;\Varid{xs}\;\Varid{k}} cannot be fully reduced. The
type of \ensuremath{\Varid{incrbyfloat}} works in a similar way.

\subsection{Disjunctive Constraints}
\label{sec:disjunctive-constraints}

Recall, from Section \ref{sec:introduction}, that commands \texttt{LPUSH key
val} and \texttt{LLEN key} return normally either when \ensuremath{\Varid{key}} presents in the
data store and is assigned a list, or when \ensuremath{\Varid{key}} does not present at all.
What we wish to have in their constraint is thus a predicate equivalent to \ensuremath{\Conid{Get}\;\Varid{xs}\;\Varid{k}\doubleequals\Conid{ListOf}\;\Varid{a}\mathrel{\vee}\neg \;(\Conid{Member}\;\Varid{xs}\;\Varid{k})}. In fact, many \Redis{} commands
are invokable under such ``well-typed, or non-existent'' precondition.

To impose a conjunctive constraint \ensuremath{\Conid{P}\mathrel{\wedge}\Conid{Q}}, one may simply put them both in the
type: \ensuremath{(\Conid{P},\Conid{Q})\Rightarrow \mathbin{...}}. Expressing disjunctive constraints is only slightly
harder, thanks to our type-level functions. We may thus write the predicate as:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Conid{Get}\;\Varid{xs}\;\Varid{k}\mathrel{\sim}\Conid{ListOf}\;\Varid{a}\mathrel{\Conid{`Or`}}\Conid{Not}\;(\Conid{Member}\;\Varid{xs}\;\Varid{k})~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
To avoid referring to \ensuremath{\Varid{a}}, which might not exist, we define an auxiliary predicate \ensuremath{\Conid{IsList}\mathbin{::}\mathbin{*}\to \Conid{Bool}} such that \ensuremath{\Conid{IsList}\;\Varid{t}} reduces to \ensuremath{\mbox{\textquotesingle}\Conid{True}}
only if \ensuremath{\Varid{t}\mathrel{=}\Conid{ListOf}\;\Varid{a}}. As many \Redis{} commands are invokable only under such
``well-typed, or non-existent'' precondition, we give names to such constraints,
as seen in Figure~\ref{fig:xxxOrNX}.

\begin{figure}[t]
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{3}{@{}>{\hspre}l<{\hspost}@{}}%
\column{5}{@{}>{\hspre}l<{\hspost}@{}}%
\column{14}{@{}>{\hspre}l<{\hspost}@{}}%
\column{18}{@{}>{\hspre}l<{\hspost}@{}}%
\column{22}{@{}>{\hspre}l<{\hspost}@{}}%
\column{24}{@{}>{\hspre}l<{\hspost}@{}}%
\column{28}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\mathbf{type}\;\Varid{family}\;\Conid{IsList}\;(\Varid{t}\mathbin{::}\mathbin{*})\mathbin{::}\Conid{Bool}\;\mathbf{where}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{IsList}\;(\Conid{ListOf}\;\Varid{a}){}\<[24]%
\>[24]{}\mathrel{=}\mbox{\textquotesingle}\Conid{True}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{IsList}\;\Varid{t}{}\<[24]%
\>[24]{}\mathrel{=}\mbox{\textquotesingle}\Conid{False}{}\<[E]%
\\
\>[B]{}\mathbf{type}\;\Varid{family}\;\Conid{IsSet}\;(\Varid{t}\mathbin{::}\mathbin{*})\mathbin{::}\Conid{Bool}\;\mathbf{where}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{IsSet}\;(\Conid{SetOf}\;\Varid{a}){}\<[22]%
\>[22]{}\mathrel{=}\mbox{\textquotesingle}\Conid{True}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{IsSet}\;\Varid{t}{}\<[22]%
\>[22]{}\mathrel{=}\mbox{\textquotesingle}\Conid{False}{}\<[E]%
\\
\>[B]{}\mathbf{type}\;\Varid{family}\;\Conid{IsString}\;(\Varid{t}\mathbin{::}\mathbin{*})\mathbin{::}\Conid{Bool}\;\mathbf{where}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{IsString}\;(\Conid{StringOf}\;\Varid{a}){}\<[28]%
\>[28]{}\mathrel{=}\mbox{\textquotesingle}\Conid{True}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{IsString}\;\Varid{t}{}\<[28]%
\>[28]{}\mathrel{=}\mbox{\textquotesingle}\Conid{False}{}\<[E]%
\\[\blanklineskip]%
\>[B]{}\mathbf{type}\;\Conid{ListOrNX}\;{}\<[18]%
\>[18]{}\Varid{xs}\;\Varid{k}\mathrel{=}{}\<[E]%
\\
\>[B]{}\hsindent{3}{}\<[3]%
\>[3]{}(\Conid{IsList}\;{}\<[14]%
\>[14]{}(\Conid{Get}\;\Varid{xs}\;\Varid{k})\mathrel{\Conid{`Or`}}\Conid{Not}\;(\Conid{Member}\;\Varid{xs}\;\Varid{k}))\mathrel{\sim}\mbox{\textquotesingle}\Conid{True}{}\<[E]%
\\
\>[B]{}\mathbf{type}\;\Conid{SetOrNX}\;{}\<[18]%
\>[18]{}\Varid{xs}\;\Varid{k}\mathrel{=}{}\<[E]%
\\
\>[B]{}\hsindent{3}{}\<[3]%
\>[3]{}(\Conid{IsSet}\;{}\<[14]%
\>[14]{}(\Conid{Get}\;\Varid{xs}\;\Varid{k})\mathrel{\Conid{`Or`}}\Conid{Not}\;(\Conid{Member}\;\Varid{xs}\;\Varid{k}))\mathrel{\sim}\mbox{\textquotesingle}\Conid{True}{}\<[E]%
\\
\>[B]{}\mathbf{type}\;\Conid{StringOrNX}\;{}\<[18]%
\>[18]{}\Varid{xs}\;\Varid{k}\mathrel{=}{}\<[E]%
\\
\>[B]{}\hsindent{3}{}\<[3]%
\>[3]{}(\Conid{IsString}\;{}\<[14]%
\>[14]{}(\Conid{Get}\;\Varid{xs}\;\Varid{k})\mathrel{\Conid{`Or`}}\Conid{Not}\;(\Conid{Member}\;\Varid{xs}\;\Varid{k}))\mathrel{\sim}\mbox{\textquotesingle}\Conid{True}{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
\caption{The ``well-typed, or non-existent'' constraints.}
\label{fig:xxxOrNX}
\end{figure}

The \Edis{} counterpart of \texttt{LPUSH} and \texttt{LLEN} are therefore:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{7}{@{}>{\hspre}l<{\hspost}@{}}%
\column{8}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{lpush}{}\<[8]%
\>[8]{}\mathbin{::}(\Conid{KnownSymbol}\;\Varid{k},\Conid{Serialize}\;\Varid{a},\Conid{ListOrNX}\;\Varid{xs}\;\Varid{k}){}\<[E]%
\\
\>[8]{}\Rightarrow \Conid{Proxy}\;\Varid{k}\to \Varid{a}\to \Conid{Edis}\;\Varid{xs}\;(\Conid{Set}\;\Varid{xs}\;\Varid{k}\;(\Conid{ListOf}\;\Varid{a}))\;(\Conid{R} \uplus \Conid{Integer}){}\<[E]%
\\
\>[B]{}\Varid{lpush}\;\Varid{key}\;\Varid{val}\mathrel{=}\Conid{Edis}\;(\Varid{\Conid{Hedis}.lpush}\;(\Varid{encodeKey}\;\Varid{key})\;[\mskip1.5mu \Varid{encode}\;\Varid{val}\mskip1.5mu])~~,{}\<[E]%
\\[\blanklineskip]%
\>[B]{}\Varid{llen}{}\<[7]%
\>[7]{}\mathbin{::}(\Conid{KnownSymbol}\;\Varid{k},\Conid{ListOrNX}\;\Varid{xs}\;\Varid{k}){}\<[E]%
\\
\>[7]{}\Rightarrow \Conid{Proxy}\;\Varid{k}\to \Conid{Edis}\;\Varid{xs}\;\Varid{xs}\;(\Conid{R} \uplus \Conid{Integer}){}\<[E]%
\\
\>[B]{}\Varid{llen}\;\Varid{key}\mathrel{=}\Conid{Edis}\;(\Varid{\Conid{Hedis}.llen}\;(\Varid{encodeKey}\;\Varid{key}))~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
Similarly, the type of \ensuremath{\Varid{sadd}}, a function we have talked about a lot,
is given below:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{7}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{sadd}{}\<[7]%
\>[7]{}\mathbin{::}(\Conid{KnownSymbol}\;\Varid{k},\Conid{Serialize}\;\Varid{a},\Conid{SetOrNX}\;\Varid{xs}\;\Varid{k}){}\<[E]%
\\
\>[7]{}\Rightarrow \Conid{Proxy}\;\Varid{k}\to \Varid{a}\to \Conid{Edis}\;\Varid{xs}\;(\Conid{Set}\;\Varid{xs}\;\Varid{k}\;(\Conid{SetOf}\;\Varid{a}))\;(\Conid{R} \uplus \Conid{Integer}){}\<[E]%
\\
\>[B]{}\Varid{sadd}\;\Varid{key}\;\Varid{val}\mathrel{=}\Conid{Edis}\;(\Varid{\Conid{Hedis}.sadd}\;(\Varid{encodeKey}\;\Varid{key})\;[\mskip1.5mu \Varid{encode}\;\Varid{val}\mskip1.5mu])~~,{}\<[E]%
\ColumnHook
\end{hscode}\resethooks

To see a command with a more complex type, consider \ensuremath{\Varid{setnx}}, which
uses the type-level function \ensuremath{\Conid{If}} defined in Section \ref{sec:type-fun}:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{8}{@{}>{\hspre}l<{\hspost}@{}}%
\column{36}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{setnx}{}\<[8]%
\>[8]{}\mathbin{::}(\Conid{KnownSymbol}\;\Varid{k},\Conid{Serialize}\;\Varid{a}){}\<[E]%
\\
\>[8]{}\Rightarrow \Conid{Proxy}\;\Varid{k}\to \Varid{a}\to \Conid{Edis}\;\Varid{xs}\;{}\<[36]%
\>[36]{}(\Conid{If}\;(\Conid{Member}\;\Varid{xs}\;\Varid{k})\;\Varid{xs}\;(\Conid{Set}\;\Varid{xs}\;\Varid{k}\;(\Conid{StringOf}\;\Varid{a})))\;{}\<[E]%
\\
\>[36]{}(\Conid{Either}\;\Conid{Reply}\;\Conid{Bool}){}\<[E]%
\\
\>[B]{}\Varid{setnx}\;\Varid{key}\;\Varid{val}\mathrel{=}\Conid{Edis}\;(\Varid{\Conid{Hedis}.setnx}\;(\Varid{encodeKey}\;\Varid{key})\;(\Varid{encode}\;\Varid{val}))~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
From the type one can see that \ensuremath{\Varid{setnx}\;\Varid{key}\;\Varid{val}} creates a new entry \ensuremath{(\Varid{key},\Varid{val})}
in the data store only if \ensuremath{\Varid{key}} is fresh. The type of \ensuremath{\Varid{setnx}} computes a
postcondition for static checking, as well as serving as a good documentation
for its semantics.

\subsection{Hashes}

{\em Hash} is a useful datatype supported by \Redis{}. While the \Redis{} data
store can be seen as a set of key/value pairs, a hash is itself a set of
field/value pairs. The following commands assigns a hash to key \texttt{user}.
The fields are \texttt{name}, \texttt{birthyear}, and \texttt{verified},
respectively with values \texttt{banacorn}, \texttt{1992}, and \texttt{1}.
\begin{Verbatim}[xleftmargin=.4in]
redis> hmset user name banacorn birthyear 1992 verified 1
OK
redis> hget user name
"banacorn"
redis> hget user birthyear
"1992"
\end{Verbatim}

For a hash to be useful, we should allow the fields to have different types. To
keep track of types of fields in a hash, \ensuremath{\Conid{HashOf}} takes a list of \ensuremath{(\Conid{Symbol},\mathbin{*})}
pairs:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\mathbf{data}\;\Conid{HashOf}\mathbin{::}[\mskip1.5mu (\Conid{Symbol},\mathbin{*})\mskip1.5mu]\to \mathbin{*}~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
By having an entry \ensuremath{(\Varid{k},\Conid{HashOF}\;\Varid{ys})} in a dictionary, we denote that the value of
key \ensuremath{\Varid{k}} is a hash whose fields and their types are specified by \ensuremath{\Varid{ys}}, which is
also a dictionary.

\begin{figure}[t]
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{5}{@{}>{\hspre}l<{\hspost}@{}}%
\column{22}{@{}>{\hspre}l<{\hspost}@{}}%
\column{34}{@{}>{\hspre}l<{\hspost}@{}}%
\column{35}{@{}>{\hspre}l<{\hspost}@{}}%
\column{36}{@{}>{\hspre}l<{\hspost}@{}}%
\column{43}{@{}>{\hspre}l<{\hspost}@{}}%
\column{44}{@{}>{\hspre}l<{\hspost}@{}}%
\column{45}{@{}>{\hspre}l<{\hspost}@{}}%
\column{76}{@{}>{\hspre}l<{\hspost}@{}}%
\column{77}{@{}>{\hspre}l<{\hspost}@{}}%
\column{81}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\mathbf{type}\;\Varid{family}\;\Conid{GetHash}\;(\Varid{xs}\mathbin{::}[\mskip1.5mu (\Conid{Symbol},\mathbin{*})\mskip1.5mu])\;(\Varid{k}\mathbin{::}\Conid{Symbol})\;(\Varid{f}\mathbin{::}\Conid{Symbol})\mathbin{::}\mathbin{*}\mathbf{where}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{GetHash}\;(\mbox{\textquotesingle}(\Varid{k},\Conid{HashOf}\;\Varid{hs}){}\<[35]%
\>[35]{}\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;{}\<[44]%
\>[44]{}\Varid{k}\;\Varid{f}\mathrel{=}\Conid{Get}\;\Varid{hs}\;\Varid{f}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{GetHash}\;(\mbox{\textquotesingle}(\Varid{l},\Varid{y}){}\<[35]%
\>[35]{}\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;{}\<[44]%
\>[44]{}\Varid{k}\;\Varid{f}\mathrel{=}\Conid{GetHash}\;\Varid{xs}\;\Varid{k}\;\Varid{f}{}\<[E]%
\\[\blanklineskip]%
\>[B]{}\mathbf{type}\;\Varid{family}\;\Conid{SetHash}\;{}\<[22]%
\>[22]{}(\Varid{xs}\mathbin{::}[\mskip1.5mu (\Conid{Symbol},\mathbin{*})\mskip1.5mu])\;(\Varid{k}\mathbin{::}\Conid{Symbol})\;{}\<[E]%
\\
\>[22]{}(\Varid{f}\mathbin{::}\Conid{Symbol})\;(\Varid{a}\mathbin{::}\mathbin{*})\mathbin{::}[\mskip1.5mu (\Conid{Symbol},\mathbin{*})\mskip1.5mu]\;\mathbf{where}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{SetHash}\;\mbox{\textquotesingle}[~]\;{}\<[44]%
\>[44]{}\Varid{k}\;\Varid{f}\;\Varid{a}\mathrel{=}\mbox{\textquotesingle}(\Varid{k},\Conid{HashOf}\;(\Conid{Set}\;\mbox{\textquotesingle}[~]\;\Varid{f}\;\Varid{a}))\mathrel{\,\mbox{\textquotesingle}\!:}\mbox{\textquotesingle}[~]{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{SetHash}\;(\mbox{\textquotesingle}(\Varid{k},\Conid{HashOf}\;\Varid{hs}){}\<[35]%
\>[35]{}\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;{}\<[44]%
\>[44]{}\Varid{k}\;\Varid{f}\;\Varid{a}\mathrel{=}\mbox{\textquotesingle}(\Varid{k},\Conid{HashOf}\;(\Conid{Set}\;\Varid{hs}\;{}\<[77]%
\>[77]{}\Varid{f}\;\Varid{a}))\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{SetHash}\;(\mbox{\textquotesingle}(\Varid{l},\Varid{y}){}\<[35]%
\>[35]{}\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;{}\<[44]%
\>[44]{}\Varid{k}\;\Varid{f}\;\Varid{a}\mathrel{=}\mbox{\textquotesingle}(\Varid{l},\Varid{y}){}\<[81]%
\>[81]{}\mathrel{\,\mbox{\textquotesingle}\!:}\Conid{SetHash}\;\Varid{xs}\;\Varid{k}\;\Varid{f}\;\Varid{a}{}\<[E]%
\\[\blanklineskip]%
\>[B]{}\mathbf{type}\;\Varid{family}\;\Conid{DelHash}\;(\Varid{xs}\mathbin{::}[\mskip1.5mu (\Conid{Symbol},\mathbin{*})\mskip1.5mu])\;(\Varid{k}\mathbin{::}\Conid{Symbol})\;(\Varid{f}\mathbin{::}\Conid{Symbol})\mathbin{::}[\mskip1.5mu (\Conid{Symbol},\mathbin{*})\mskip1.5mu]\;\mathbf{where}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{DelHash}\;\mbox{\textquotesingle}[~]\;{}\<[43]%
\>[43]{}\Varid{k}\;\Varid{f}\mathrel{=}\mbox{\textquotesingle}[~]{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{DelHash}\;(\mbox{\textquotesingle}(\Varid{k},\Conid{HashOf}\;\Varid{hs})\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;{}\<[43]%
\>[43]{}\Varid{k}\;\Varid{f}\mathrel{=}\mbox{\textquotesingle}(\Varid{k},\Conid{HashOf}\;(\Conid{Del}\;\Varid{hs}\;\Varid{f}))\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{DelHash}\;(\mbox{\textquotesingle}(\Varid{l},\Varid{y}){}\<[34]%
\>[34]{}\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;{}\<[43]%
\>[43]{}\Varid{k}\;\Varid{f}\mathrel{=}\mbox{\textquotesingle}(\Varid{l},\Varid{y}){}\<[76]%
\>[76]{}\mathrel{\,\mbox{\textquotesingle}\!:}\Conid{DelHash}\;\Varid{xs}\;\Varid{k}\;\Varid{f}{}\<[E]%
\\[\blanklineskip]%
\>[B]{}\mathbf{type}\;\Varid{family}\;\Conid{MemHash}\;(\Varid{xs}\mathbin{::}[\mskip1.5mu (\Conid{Symbol},\mathbin{*})\mskip1.5mu])\;(\Varid{k}\mathbin{::}\Conid{Symbol})\;(\Varid{f}\mathbin{::}\Conid{Symbol})\mathbin{::}\Conid{Bool}\;\mathbf{where}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{MemHash}\;\mbox{\textquotesingle}[~]\;{}\<[45]%
\>[45]{}\Varid{k}\;\Varid{f}\mathrel{=}\mbox{\textquotesingle}\Conid{False}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{MemHash}\;(\mbox{\textquotesingle}(\Varid{k},\Conid{HashOf}\;\Varid{hs}){}\<[36]%
\>[36]{}\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;{}\<[45]%
\>[45]{}\Varid{k}\;\Varid{f}\mathrel{=}\Conid{Member}\;\Varid{hs}\;\Varid{f}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{MemHash}\;(\mbox{\textquotesingle}(\Varid{k},\Varid{x}){}\<[36]%
\>[36]{}\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;{}\<[45]%
\>[45]{}\Varid{k}\;\Varid{f}\mathrel{=}\mbox{\textquotesingle}\Conid{False}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{MemHash}\;(\mbox{\textquotesingle}(\Varid{l},\Varid{y}){}\<[36]%
\>[36]{}\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;{}\<[45]%
\>[45]{}\Varid{k}\;\Varid{f}\mathrel{=}\Conid{MemHash}\;\Varid{xs}\;\Varid{k}\;\Varid{f}{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
\caption{Type-level operations for dictionaries with hashes.}
\label{fig:xxxHash}
\end{figure}

Figure \ref{fig:xxxHash} presents some operations we need on dictionaries when
dealing with hashes. Let \ensuremath{\Varid{xs}} be a dictionary, \ensuremath{\Conid{GetHash}\;\Varid{xs}\;\Varid{k}\;\Varid{f}} returns the type
of field \ensuremath{\Varid{f}} in the hash assigned to key \ensuremath{\Varid{k}}, if both \ensuremath{\Varid{k}} and \ensuremath{\Varid{f}} exists.
\ensuremath{\Conid{SetHash}\;\Varid{xs}\;\Varid{k}\;\Varid{f}\;\Varid{a}} assigns the type \ensuremath{\Varid{a}} to the field \ensuremath{\Varid{f}} of hash \ensuremath{\Varid{k}}; if either
\ensuremath{\Varid{f}} or \ensuremath{\Varid{k}} does not exist, the hash/field is created. \ensuremath{\Conid{Del}\;\Varid{xs}\;\Varid{k}\;\Varid{f}} removes a
field, while \ensuremath{\Conid{MemHash}\;\Varid{xs}\;\Varid{k}\;\Varid{f}} checks whether the key \ensuremath{\Varid{k}} exists in \ensuremath{\Varid{xs}}, and its
value is a hash having field \ensuremath{\Varid{f}}. Their definitions make use of functions \ensuremath{\Conid{Get}},
\ensuremath{\Conid{Set}}, and \ensuremath{\Conid{Member}} defined for dictionaries.

Once those type-level functions are defined, embedding of \Hedis{} commands for
hashes is more or less routine. For example, functions \ensuremath{\Varid{hset}} and \ensuremath{\Varid{hget}}
are shown below. Note that, instead of \ensuremath{\Varid{hmset}} (available in \Hedis{}), we
provide a function \ensuremath{\Varid{hset}} that assigns fields and values one pair at a time.
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{3}{@{}>{\hspre}l<{\hspost}@{}}%
\column{7}{@{}>{\hspre}l<{\hspost}@{}}%
\column{13}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{hset}{}\<[7]%
\>[7]{}\mathbin{::}(\Conid{KnownSymbol}\;\Varid{k},\Conid{KnownSymbol}\;\Varid{f},\Conid{Serialize}\;\Varid{a},\Conid{HashOrNX}\;\Varid{xs}\;\Varid{k}){}\<[E]%
\\
\>[7]{}\Rightarrow \Conid{Proxy}\;\Varid{k}\to \Conid{Proxy}\;\Varid{f}\to \Varid{a}{}\<[E]%
\\
\>[7]{}\to \Conid{Edis}\;\Varid{xs}\;(\Conid{SetHash}\;\Varid{xs}\;\Varid{k}\;\Varid{f}\;(\Conid{StringOf}\;\Varid{a}))\;(\Conid{R} \uplus \Conid{Bool}){}\<[E]%
\\
\>[B]{}\Varid{hset}\;\Varid{key}\;\Varid{field}\;\Varid{val}\mathrel{=}{}\<[E]%
\\
\>[B]{}\hsindent{3}{}\<[3]%
\>[3]{}\Conid{Edis}\;(\Varid{\Conid{Hedis}.hset}\;(\Varid{encodeKey}\;\Varid{key})\;(\Varid{encodeKey}\;\Varid{field})\;(\Varid{encode}\;\Varid{val}))~~,{}\<[E]%
\\[\blanklineskip]%
\>[B]{}\Varid{hget}{}\<[7]%
\>[7]{}\mathbin{::}({}\<[13]%
\>[13]{}\Conid{KnownSymbol}\;\Varid{k},\Conid{KnownSymbol}\;\Varid{f},\Conid{Serialize}\;\Varid{a},{}\<[E]%
\\
\>[13]{}\Conid{StringOf}\;\Varid{a}\mathrel{\sim}\Conid{GetHash}\;\Varid{xs}\;\Varid{k}\;\Varid{f}){}\<[E]%
\\
\>[7]{}\Rightarrow \Conid{Proxy}\;\Varid{k}\to \Conid{Proxy}\;\Varid{f}\to \Conid{Edis}\;\Varid{xs}\;\Varid{xs}\;(\Conid{R} \uplus \Conid{Maybe}\;\Varid{a}){}\<[E]%
\\
\>[B]{}\Varid{hget}\;\Varid{key}\;\Varid{field}\mathrel{=}{}\<[E]%
\\
\>[B]{}\hsindent{3}{}\<[3]%
\>[3]{}\Conid{Edis}\;(\Varid{\Conid{Hedis}.hget}\;(\Varid{encodeKey}\;\Varid{key})\;(\Varid{encodeKey}\;\Varid{field})\bind \Varid{decodeAsMaybe})~~,{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
where \ensuremath{\Varid{decodeAsMaybe}\mathbin{::}\Conid{Serialize}\;\Varid{a}\Rightarrow (\Conid{R} \uplus \Conid{Maybe}\;\Conid{ByteString})\to \Conid{Redis}\;(\Conid{R} \uplus \Conid{Maybe}\;\Varid{a})}, using the function \ensuremath{\Varid{decode}}
mentioned in Section \ref{sec:proxy-key}, parses the \ensuremath{\Conid{ByteString}} in
\ensuremath{\Conid{R} \uplus \Conid{Maybe}\;\anonymous } to type \ensuremath{\Varid{a}}. The definition is a bit tedious but
routine.

Note that, instead of \ensuremath{\Varid{hmset}} (available in \Hedis{}), we
provide a function \ensuremath{\Varid{hset}} that assigns fields and values one pair at at time.
We will talk about difficulties of implementing \ensuremath{\Varid{hmset}} in
Section~\ref{sec:discussions}.

\subsection{Assertions}
\label{sec:assertions}

% Consider the following scenario: We want to retrieve the value of some existing
% key, say, |"ab initio"|, with the function\footnote{The semantics of |get| in
% \Redis{} is actually more forgiving. See Section~\ref{sec:discussions}.}:
% \begin{spec}
% get  :: (KnownSymbol k, Serialize a, StringOf a ~ Get xs k)
%      => Proxy k -> Edis xs xs (EitherReply (Maybe a)) {-"~~."-}
% \end{spec}
%
% However, Haskell would complain that, the key |"ab initio"| was not
% before seen in the dictionary. So we could never write programs to retrieve the
% value of |"ab initio"|, unless its creation was witnessed by the type checker.


Finally, the creation/update behavior of \Redis{} functions is, in our opinion,
very error-prone. It might be preferable if we can explicit declare some new
keys, after ensuring that they do not already exist (in our types). This can be done below:
% It might be preferable if we can explicitly declare some new keys, under the
%  precondition that they do not already exist in our types. This can be done as
%  follows:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{10}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{declare}{}\<[10]%
\>[10]{}\mathbin{::}(\Conid{KnownSymbol}\;\Varid{k},\Conid{Member}\;\Varid{xs}\;\Varid{k}\mathrel{\sim}\Conid{False}){}\<[E]%
\\
\>[10]{}\Rightarrow \Conid{Proxy}\;\Varid{k}\to \Conid{Proxy}\;\Varid{a}\to \Conid{Edis}\;\Varid{xs}\;(\Conid{Set}\;\Varid{xs}\;\Varid{k}\;\Varid{a})\;(){}\<[E]%
\\
\>[B]{}\Varid{declare}\;\Varid{key}\;\Varid{typ}\mathrel{=}\Conid{Edis}\;(\Varid{return}\;())~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
% renounce :: (KnownSymbol s, Member xs s ~ True)
%         => Proxy s -> Edis xs (Del xs s) ()
% renounce s = Edis $ return () {-"~~."-}
The command \ensuremath{\Varid{declare}\;\Varid{key}\;\Varid{typ}}, where \ensuremath{\Varid{typ}} is the proxy of \ensuremath{\Varid{a}}, adds a fresh
 \ensuremath{\Varid{key}} with type \ensuremath{\Varid{a}} into the dictionary. Notice that \ensuremath{\Varid{declare}} does nothing at
 term level, but simply returns \ensuremath{()}, since it only has effects on types.

% The key is not actually created yet.
% The declaration, however, ensures that if |key| is actually created, perhaps
% by one of those ``well-typed or non-existent'' command, its type must be |a|.
% The command |start| initializes the dictionary to the empty list:

Another command for type level assertion, \ensuremath{\Varid{start}}, initializes the dictionary to
 the empty list, comes in handy when starting a series of \Edis{} commands:

\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{start}\mathbin{::}\Conid{Edis}\;\mbox{\textquotesingle}[~]\;\mbox{\textquotesingle}[~]\;(){}\<[E]%
\\
\>[B]{}\Varid{start}\mathrel{=}\Conid{Edis}\;(\Varid{return}\;())~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks

\subsection{A Larger Example}

We present a larger example as a summary. The task is to store a queue of
messages in \Redis{}. Messages are represented by a \ensuremath{\Conid{ByteString}} and an
\ensuremath{\Conid{Integer}} identifier:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{35}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\mathbf{data}\;\Conid{Message}\mathrel{=}\Conid{Msg}\;\Conid{ByteString}\;\Conid{Integer}\;\mathbf{deriving}\;(\Conid{Show},\Conid{Generic})~~,{}\<[E]%
\\
\>[B]{}\mathbf{instance}\;\Conid{Serialize}\;\Conid{Message}\;\mathbf{where}\;{}\<[35]%
\>[35]{}~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks

In the data store, the queue is represented by a list. Before pushing a message
into the queue, we increment \ensuremath{\Varid{counter}}, a key storing a counter, and use it as the
identifier of the message:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{5}{@{}>{\hspre}l<{\hspost}@{}}%
\column{7}{@{}>{\hspre}l<{\hspost}@{}}%
\column{13}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{push}{}\<[7]%
\>[7]{}\mathbin{::}(\Conid{StringOfIntegerOrNX}\;\Varid{xs}\;\text{\tt \char34 counter\char34},\Conid{ListOrNX}\;\Varid{xs}\;\text{\tt \char34 queue\char34}){}\<[E]%
\\
\>[7]{}\Rightarrow \Conid{ByteString}\to \Conid{Edis}\;\Varid{xs}\;(\Conid{Set}\;\Varid{xs}\;\text{\tt \char34 queue\char34}\;(\Conid{ListOf}\;\Conid{Message}))\;(\Conid{R} \uplus \Conid{Integer}){}\<[E]%
\\
\>[B]{}\Varid{push}\;\Varid{msg}\mathrel{=}{}\<[13]%
\>[13]{}\Varid{incr}\;\Varid{kCounter}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\mathbin{`\Varid{bind}`}{}\<[13]%
\>[13]{}\lambda \Varid{i}\to \Varid{lpush}\;\Varid{kQueue}\;(\Conid{Msg}\;\Varid{msg}\;(\Varid{fromRight}\;\Varid{i}))~~,{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
%​
where \ensuremath{\Varid{fromRight}\mathbin{::}\Conid{Either}\;\Varid{a}\;\Varid{b}\to \Varid{b}} extracts the value wrapped by constructor
\ensuremath{\Conid{Right}}, and the constraint \ensuremath{\Conid{StringOfIntegerOrNX}\;\Varid{xs}\;\Varid{k}} holds if either \ensuremath{\Varid{k}}
presents in \ensuremath{\Varid{xs}} and is converted from an \ensuremath{\Conid{Integer}}, or \ensuremath{\Varid{k}} does not
present in \ensuremath{\Varid{xs}}. For brevity, the proxies are given names: \\
\noindent{\centering %\small
\begin{minipage}[b]{0.4\linewidth}
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{14}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{kCounter}\mathbin{::}{}\<[14]%
\>[14]{}\Conid{Proxy}\;\text{\tt \char34 counter\char34}{}\<[E]%
\\
\>[B]{}\Varid{kCounter}\mathrel{=}{}\<[14]%
\>[14]{}\Conid{Proxy}~~,{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
\end{minipage}
\begin{minipage}[b]{0.4\linewidth}
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{12}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{kQueue}\mathbin{::}{}\<[12]%
\>[12]{}\Conid{Proxy}\;\text{\tt \char34 queue\char34}{}\<[E]%
\\
\>[B]{}\Varid{kQueue}\mathrel{=}{}\<[12]%
\>[12]{}\Conid{Proxy}~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
\end{minipage}}\\
To pop a message we use the function \ensuremath{\Varid{rpop}} which, given a key associated with
a list, extracts the rightmost element of the list
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{6}{@{}>{\hspre}l<{\hspost}@{}}%
\column{7}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{pop}{}\<[6]%
\>[6]{}\mathbin{::}(\Conid{Get}\;\Varid{xs}\;\text{\tt \char34 queue\char34}\mathrel{\sim}\Conid{ListOf}\;\Conid{Message}){}\<[E]%
\\
\>[6]{}\Rightarrow \Conid{Edis}\;\Varid{xs}\;\Varid{xs}\;(\Conid{R} \uplus \Conid{Maybe}\;\Conid{Message}){}\<[E]%
\\
\>[B]{}\Varid{pop}\mathrel{=}\Varid{rpop}\;\Varid{kQueue}~~,{}\<[E]%
\\[\blanklineskip]%
\>[B]{}\Varid{rpop}{}\<[7]%
\>[7]{}\mathbin{::}(\Conid{KnownSymbol}\;\Varid{k},\Conid{Serialize}\;\Varid{a},\Conid{Get}\;\Varid{xs}\;\Varid{k}\mathrel{\sim}\Conid{ListOf}\;\Varid{a}){}\<[E]%
\\
\>[7]{}\Rightarrow \Conid{Proxy}\;\Varid{k}\to \Conid{Edis}\;\Varid{xs}\;\Varid{xs}\;(\Conid{R} \uplus \Conid{Maybe}\;\Varid{a}){}\<[E]%
\\
\>[B]{}\Varid{rpop}\;\Varid{key}\mathrel{=}\Conid{Edis}\;(\Varid{\Conid{Hedis}.rpop}\;(\Varid{encodeKey}\;\Varid{key})\bind \Varid{decodeAsMaybe})~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
To get things going, the main program builds a connection with the \Redis{}
server, runs an embedded program \ensuremath{\Varid{prog}}, and prints the result, which in this
example is \ensuremath{\text{\tt \char34 hello\char34}}:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{4}{@{}>{\hspre}c<{\hspost}@{}}%
\column{4E}{@{}l@{}}%
\column{9}{@{}>{\hspre}l<{\hspost}@{}}%
\column{12}{@{}>{\hspre}l<{\hspost}@{}}%
\column{20}{@{}>{\hspre}l<{\hspost}@{}}%
\column{27}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{main}\mathbin{::}\Conid{IO}\;(){}\<[E]%
\\
\>[B]{}\Varid{main}\mathrel{=}\mathbf{do}\;{}\<[12]%
\>[12]{}\Varid{conn}{}\<[20]%
\>[20]{}\leftarrow \Varid{connect}\;\Varid{defaultConnectInfo}{}\<[E]%
\\
\>[12]{}\Varid{result}{}\<[20]%
\>[20]{}\leftarrow \Varid{runRedis}\;\Varid{conn}\;(\Varid{unEdis}\;(\Varid{start}\mathbin{>\!\!\!>\!\!\!>}\Varid{prog})){}\<[E]%
\\
\>[12]{}\Varid{print}\;\Varid{result}~~,{}\<[E]%
\\[\blanklineskip]%
\>[B]{}\Varid{prog}\mathrel{=}{}\<[9]%
\>[9]{}\Varid{declare}\;\Varid{kCounter}\;{}\<[27]%
\>[27]{}(\Conid{Proxy}\mathbin{::}\Conid{Proxy}\;\Conid{Integer}){}\<[E]%
\\
\>[B]{}\hsindent{4}{}\<[4]%
\>[4]{}\mathbin{>\!\!\!>\!\!\!>}{}\<[4E]%
\>[9]{}\Varid{declare}\;\Varid{kQueue}\;{}\<[27]%
\>[27]{}(\Conid{Proxy}\mathbin{::}\Conid{Proxy}\;(\Conid{ListOf}\;\Conid{Message})){}\<[E]%
\\
\>[B]{}\hsindent{4}{}\<[4]%
\>[4]{}\mathbin{>\!\!\!>\!\!\!>}{}\<[4E]%
\>[9]{}\Varid{push}\;\text{\tt \char34 hello\char34}{}\<[E]%
\\
\>[B]{}\hsindent{4}{}\<[4]%
\>[4]{}\mathbin{>\!\!\!>\!\!\!>}{}\<[4E]%
\>[9]{}\Varid{push}\;\text{\tt \char34 world\char34}{}\<[E]%
\\
\>[B]{}\hsindent{4}{}\<[4]%
\>[4]{}\mathbin{>\!\!\!>\!\!\!>}{}\<[4E]%
\>[9]{}\Varid{pop}~~,{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
where the monadic sequencing operator \ensuremath{(\mathbin{>\!\!\!>\!\!\!>})} is defined by:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}(\mathbin{>\!\!\!>\!\!\!>})\mathbin{::}\Conid{IMonad}\;\Varid{m}\Rightarrow \Varid{m}\;\Varid{p}\;\Varid{q}\;\Varid{a}\to \Varid{m}\;\Varid{q}\;\Varid{r}\;\Varid{b}\to \Varid{m}\;\Varid{p}\;\Varid{r}\;\Varid{b}{}\<[E]%
\\
\>[B]{}\Varid{m}_{1}\mathbin{>\!\!\!>\!\!\!>}\Varid{m}_{2}\mathrel{=}\Varid{m}_{1}\mathbin{`\Varid{bind}`}(\lambda \anonymous \to \Varid{m}_{2})~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
Use of \ensuremath{\Varid{declare}} in \ensuremath{\Varid{prog}} ensures that neither \ensuremath{\text{\tt \char34 counter\char34}} nor \ensuremath{\text{\tt \char34 queue\char34}} exist
before the execution of \ensuremath{\Varid{prog}}, while \ensuremath{\Varid{start}} in \ensuremath{\Varid{main}} guarantees that the
program is given a fresh run without previously defined keys at all. Haskell
is able to infer the type of \ensuremath{\Varid{prog}}:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{15}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{prog}\mathbin{::}\Conid{Edis}\;{}\<[15]%
\>[15]{}\mbox{\textquotesingle}[~]\;\mbox{\textquotesingle}[\mbox{\textquotesingle}(\text{\tt \char34 counter\char34},\Conid{Integer}),\mbox{\textquotesingle}(\text{\tt \char34 queue\char34},\Conid{ListOf}\;\Conid{Message})]\;{}\<[E]%
\\
\>[15]{}(\Conid{R} \uplus \Conid{Maybe}\;\Conid{Message})~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks


% The following program increases the value of |"A"| as an integer, push the result of the increment to list |"L"|, and then pops it out:
% \begin{spec}
% main :: IO ()
% main = do
%     conn    <- connect defaultConnectInfo
%     result  <- runRedis conn $ unEdis $ start
%         `bind` \ _ ->  declare (Proxy :: Proxy "A") (Proxy :: Proxy Integer)
%         `bind` \ _ ->  incr (Proxy :: Proxy "A")
%         `bind` \n ->  case n of
%             Left  err  -> lpush (Proxy :: Proxy "L") 0
%             Right n    -> lpush (Proxy :: Proxy "L") n
%         `bind` \ _ ->  lpop     (Proxy :: Proxy "L")
%     print result
% \end{spec}

% The syntax is pretty heavy, like the old days when there's no
%  \emph{do-notation}\cite{history}. But if we don't need any variable bindings
%  between operations, we could compose these commands with a sequencing operator
%  |(>>>)|.


% \begin{spec}
% program = start
%     >>> declare (Proxy :: Proxy "A") (Proxy :: Proxy Integer)
%     >>> incr    (Proxy :: Proxy "A")
%     >>> lpush   (Proxy :: Proxy "L") 0
%     >>> lpop    (Proxy :: Proxy "L")
% \end{spec}


==> sections/IndexedMonads.tex <==
%% ODER: format ==         = "\mathrel{==}"
%% ODER: format /=         = "\neq "
%
%
\makeatletter
\@ifundefined{lhs2tex.lhs2tex.sty.read}%
  {\@namedef{lhs2tex.lhs2tex.sty.read}{}%
   \newcommand\SkipToFmtEnd{}%
   \newcommand\EndFmtInput{}%
   \long\def\SkipToFmtEnd#1\EndFmtInput{}%
  }\SkipToFmtEnd

\newcommand\ReadOnlyOnce[1]{\@ifundefined{#1}{\@namedef{#1}{}}\SkipToFmtEnd}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{stmaryrd}
\DeclareFontFamily{OT1}{cmtex}{}
\DeclareFontShape{OT1}{cmtex}{m}{n}
  {<5><6><7><8>cmtex8
   <9>cmtex9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmtex10}{}
\DeclareFontShape{OT1}{cmtex}{m}{it}
  {<-> ssub * cmtt/m/it}{}
\newcommand{\texfamily}{\fontfamily{cmtex}\selectfont}
\DeclareFontShape{OT1}{cmtt}{bx}{n}
  {<5><6><7><8>cmtt8
   <9>cmbtt9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmbtt10}{}
\DeclareFontShape{OT1}{cmtex}{bx}{n}
  {<-> ssub * cmtt/bx/n}{}
\newcommand{\tex}[1]{\text{\texfamily#1}}	% NEU

\newcommand{\Sp}{\hskip.33334em\relax}


\newcommand{\Conid}[1]{\mathit{#1}}
\newcommand{\Varid}[1]{\mathit{#1}}
\newcommand{\anonymous}{\kern0.06em \vbox{\hrule\@width.5em}}
\newcommand{\plus}{\mathbin{+\!\!\!+}}
\newcommand{\bind}{\mathbin{>\!\!\!>\mkern-6.7mu=}}
\newcommand{\rbind}{\mathbin{=\mkern-6.7mu<\!\!\!<}}% suggested by Neil Mitchell
\newcommand{\sequ}{\mathbin{>\!\!\!>}}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\usepackage{polytable}

%mathindent has to be defined
\@ifundefined{mathindent}%
  {\newdimen\mathindent\mathindent\leftmargini}%
  {}%

\def\resethooks{%
  \global\let\SaveRestoreHook\empty
  \global\let\ColumnHook\empty}
\newcommand*{\savecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\savecolumns[#1]}}
\newcommand*{\restorecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\restorecolumns[#1]}}
\newcommand*{\aligncolumn}[2]%
  {\g@addto@macro\ColumnHook{\column{#1}{#2}}}

\resethooks

\newcommand{\onelinecommentchars}{\quad-{}- }
\newcommand{\commentbeginchars}{\enskip\{-}
\newcommand{\commentendchars}{-\}\enskip}

\newcommand{\visiblecomments}{%
  \let\onelinecomment=\onelinecommentchars
  \let\commentbegin=\commentbeginchars
  \let\commentend=\commentendchars}

\newcommand{\invisiblecomments}{%
  \let\onelinecomment=\empty
  \let\commentbegin=\empty
  \let\commentend=\empty}

\visiblecomments

\newlength{\blanklineskip}
\setlength{\blanklineskip}{0.66084ex}

\newcommand{\hsindent}[1]{\quad}% default is fixed indentation
\let\hspre\empty
\let\hspost\empty
\newcommand{\NB}{\textbf{NB}}
\newcommand{\Todo}[1]{$\langle$\textbf{To do:}~#1$\rangle$}

\EndFmtInput
\makeatother
%
%
%
%
%
%
% This package provides two environments suitable to take the place
% of hscode, called "plainhscode" and "arrayhscode". 
%
% The plain environment surrounds each code block by vertical space,
% and it uses \abovedisplayskip and \belowdisplayskip to get spacing
% similar to formulas. Note that if these dimensions are changed,
% the spacing around displayed math formulas changes as well.
% All code is indented using \leftskip.
%
% Changed 19.08.2004 to reflect changes in colorcode. Should work with
% CodeGroup.sty.
%
\ReadOnlyOnce{polycode.fmt}%
\makeatletter

\newcommand{\hsnewpar}[1]%
  {{\parskip=0pt\parindent=0pt\par\vskip #1\noindent}}

% can be used, for instance, to redefine the code size, by setting the
% command to \small or something alike
\newcommand{\hscodestyle}{}

% The command \sethscode can be used to switch the code formatting
% behaviour by mapping the hscode environment in the subst directive
% to a new LaTeX environment.

\newcommand{\sethscode}[1]%
  {\expandafter\let\expandafter\hscode\csname #1\endcsname
   \expandafter\let\expandafter\endhscode\csname end#1\endcsname}

% "compatibility" mode restores the non-polycode.fmt layout.

\newenvironment{compathscode}%
  {\par\noindent
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \let\hspre\(\let\hspost\)%
   \pboxed}%
  {\endpboxed\)%
   \par\noindent
   \ignorespacesafterend}

\newcommand{\compaths}{\sethscode{compathscode}}

% "plain" mode is the proposed default.
% It should now work with \centering.
% This required some changes. The old version
% is still available for reference as oldplainhscode.

\newenvironment{plainhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\hspre\(\let\hspost\)%
   \pboxed}%
  {\endpboxed%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

\newenvironment{oldplainhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

% Here, we make plainhscode the default environment.

\newcommand{\plainhs}{\sethscode{plainhscode}}
\newcommand{\oldplainhs}{\sethscode{oldplainhscode}}
\plainhs

% The arrayhscode is like plain, but makes use of polytable's
% parray environment which disallows page breaks in code blocks.

\newenvironment{arrayhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\parray}%
  {\endparray\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

\newcommand{\arrayhs}{\sethscode{arrayhscode}}

% The mathhscode environment also makes use of polytable's parray 
% environment. It is supposed to be used only inside math mode 
% (I used it to typeset the type rules in my thesis).

\newenvironment{mathhscode}%
  {\parray}{\endparray}

\newcommand{\mathhs}{\sethscode{mathhscode}}

% texths is similar to mathhs, but works in text mode.

\newenvironment{texthscode}%
  {\(\parray}{\endparray\)}

\newcommand{\texths}{\sethscode{texthscode}}

% The framed environment places code in a framed box.

\def\codeframewidth{\arrayrulewidth}
\RequirePackage{calc}

\newenvironment{framedhscode}%
  {\parskip=\abovedisplayskip\par\noindent
   \hscodestyle
   \arrayrulewidth=\codeframewidth
   \tabular{@{}|p{\linewidth-2\arraycolsep-2\arrayrulewidth-2pt}|@{}}%
   \hline\framedhslinecorrect\\{-1.5ex}%
   \let\endoflinesave=\\
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \framedhslinecorrect\endoflinesave{.5ex}\hline
   \endtabular
   \parskip=\belowdisplayskip\par\noindent
   \ignorespacesafterend}

\newcommand{\framedhslinecorrect}[2]%
  {#1[#2]}

\newcommand{\framedhs}{\sethscode{framedhscode}}

% The inlinehscode environment is an experimental environment
% that can be used to typeset displayed code inline.

\newenvironment{inlinehscode}%
  {\(\def\column##1##2{}%
   \let\>\undefined\let\<\undefined\let\\\undefined
   \newcommand\>[1][]{}\newcommand\<[1][]{}\newcommand\\[1][]{}%
   \def\fromto##1##2##3{##3}%
   \def\nextline{}}{\) }%

\newcommand{\inlinehs}{\sethscode{inlinehscode}}

% The joincode environment is a separate environment that
% can be used to surround and thereby connect multiple code
% blocks.

\newenvironment{joincode}%
  {\let\orighscode=\hscode
   \let\origendhscode=\endhscode
   \def\endhscode{\def\hscode{\endgroup\def\@currenvir{hscode}\\}\begingroup}
   %\let\SaveRestoreHook=\empty
   %\let\ColumnHook=\empty
   %\let\resethooks=\empty
   \orighscode\def\hscode{\endgroup\def\@currenvir{hscode}}}%
  {\origendhscode
   \global\let\hscode=\orighscode
   \global\let\endhscode=\origendhscode}%

\makeatother
\EndFmtInput
%

\ReadOnlyOnce{Formatting.fmt}%
\makeatletter

\let\Varid\mathit
\let\Conid\mathsf

\def\commentbegin{\quad\{\ }
\def\commentend{\}}

\newcommand{\ty}[1]{\Conid{#1}}
\newcommand{\con}[1]{\Conid{#1}}
\newcommand{\id}[1]{\Varid{#1}}
\newcommand{\cl}[1]{\Varid{#1}}
\newcommand{\opsym}[1]{\mathrel{#1}}

\newcommand\Keyword[1]{\textbf{\textsf{#1}}}
\newcommand\Hide{\mathbin{\downarrow}}
\newcommand\Reveal{\mathbin{\uparrow}}


%% Paper-specific keywords


\makeatother
\EndFmtInput

\section{Indexed Monads}
\label{sec:indexed-monads}

Stateful computations are often reasoned using Hoare logic. A {\em Hoare triple}
$\{P\} S \{Q\}$ denotes the following proposition: if the statement $S$ is
executed in a state satisfying predicate $P$, when it terminates, the state must
satisfy predicate $Q$. Predicates $P$ and $Q$ are respectively called the
\emph{precondition} and the \emph{postcondition} of the Hoare triple.

In Haskell, stateful computations are represented by monads. To reason about
them within the type system, we wish to label a state monad with its pre and
postcondition. An \emph{indexed monad}~\cite{indexedmonad} (also called a
\emph{parameterised monad} or \emph{monadish}) is a monad that, in addition to
the type of its result, takes two more type parameters representing an initial
state and a final state, to be interpreted like a Hoare triple:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{5}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\mathbf{class}\;\Conid{IMonad}\;\Varid{m}\;\mathbf{where}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Varid{unit}\mathbin{::}\Varid{a}\to \Varid{m}\;\Varid{p}\;\Varid{p}\;\Varid{a}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Varid{bind}\mathbin{::}\Varid{m}\;\Varid{p}\;\Varid{q}\;\Varid{a}\to (\Varid{a}\to \Varid{m}\;\Varid{q}\;\Varid{r}\;\Varid{b})\to \Varid{m}\;\Varid{p}\;\Varid{r}\;\Varid{b}~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
The intention is that a computation of type \ensuremath{\Varid{m}\;\Varid{p}\;\Varid{q}\;\Varid{a}} is a stateful computation
such that, if it starts execution in a state satisfying \ensuremath{\Varid{p}} and terminates, it
yields a value of type \ensuremath{\Varid{a}}, and the new state satisfies \ensuremath{\Varid{q}}. The operator \ensuremath{\Varid{unit}}
lifts a pure computation to a stateful computation that does not alter the
state. In \ensuremath{\Varid{x}\mathbin{`\Varid{bind}`}\Varid{f}}, a computation \ensuremath{\Varid{x}\mathbin{::}\Varid{m}\;\Varid{p}\;\Varid{q}\;\Varid{a}} is followed by
\ensuremath{\Varid{f}\mathbin{::}\Varid{a}\to \Varid{m}\;\Varid{q}\;\Varid{r}\;\Varid{b}} --- the postcondition of \ensuremath{\Varid{x}} matches the precondition of
the computation returned by \ensuremath{\Varid{f}}. The result is a computation \ensuremath{\Varid{m}\;\Varid{p}\;\Varid{r}\;\Varid{b}}.

We define a new indexed monad \ensuremath{\Conid{Edis}}. At term level, the \ensuremath{\Varid{unit}} and \ensuremath{\Varid{bind}}
methods are not interesting: they merely make calls to \ensuremath{\Varid{return}} and \ensuremath{(\mathbin{>\!\!>\!\!=})} of
\ensuremath{\Conid{Redis}}, and extract and re-apply the constructor \ensuremath{\Conid{Edis}} when necessary.
With \ensuremath{\Conid{Edis}} being a \ensuremath{\mathbf{newtype}}, they can be optimized away in runtime. The
purpose is to add the pre/postconditions at type level:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{5}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\mathbf{newtype}\;\Conid{Edis}\;\Varid{p}\;\Varid{q}\;\Varid{a}\mathrel{=}\Conid{Edis}\;\{\mskip1.5mu \Varid{unEdis}\mathbin{::}\Conid{Redis}\;\Varid{a}\mskip1.5mu\}~~,{}\<[E]%
\\[\blanklineskip]%
\>[B]{}\mathbf{instance}\;\Conid{IMonad}\;\Conid{Edis}\;\mathbf{where}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Varid{unit}\mathrel{=}\Conid{Edis}\mathbin{\cdot}\Varid{return}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Varid{bind}\;\Varid{m}\;\Varid{f}\mathrel{=}\Conid{Edis}\;(\Varid{unEdis}\;\Varid{m}\mathbin{>\!\!>\!\!=}\Varid{unEdis}\mathbin{\cdot}\Varid{f})~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks

The properties of the state we care about are the set of currently
allocated keys and types of their values. We will present, in Section~\ref{sec:type-level-dict}, techniques that allow us to specify
properties such as ``the keys in the data store are \ensuremath{\text{\tt \char34 A\char34}}, \ensuremath{\text{\tt \char34 B\char34}}, and \ensuremath{\text{\tt \char34 C\char34}},
respectively assigned values of type \ensuremath{\Conid{Int}}, \ensuremath{\Conid{Char}}, and \ensuremath{\Conid{Bool}}.'' For now,
however, let us look at the simplest \Redis{} command.

\Redis{} commands can be executed in two contexts: the normal context, or a \emph{transaction}. In \Hedis{}, a command yielding value of type \ensuremath{\Varid{a}} in the
normal case is represented by \ensuremath{\Conid{Redis}\;(\Conid{Either}\;\Conid{Reply}\;\Varid{a})}, as mentioned in
Section~\ref{sec:introduction}; in a transaction, the command is represented by
two other datatypes \ensuremath{\Conid{RedisTx}\;(\Conid{Queued}\;\Varid{a})}. In this paper we focus on the former
case. For brevity we abbreviate \ensuremath{\Conid{Either}\;\Conid{Reply}\;\Varid{a}} to \ensuremath{\Conid{R} \uplus \Varid{a}}.

The command \texttt{PING} in \Redis{} does nothing but replying a message
\texttt{PONG} if the connection is alive. In \Hedis{}, \ensuremath{\Varid{ping}} has type
\ensuremath{\Conid{Redis}\;(\Conid{R} \uplus \Conid{Status})}. The \Edis{} version of \ensuremath{\Varid{ping}} simply applies an additional constructor (functions from \Hedis{} are qualified with \ensuremath{\Conid{Hedis}} to
prevent name clashing):
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{ping}\mathbin{::}\Conid{Edis}\;\Varid{xs}\;\Varid{xs}\;(\Conid{R} \uplus \Conid{Status}){}\<[E]%
\\
\>[B]{}\Varid{ping}\mathrel{=}\Conid{Edis}\;\Varid{\Conid{Hedis}.ping}~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
Since \ensuremath{\Varid{ping}} does not alter the data store, the postcondition and precondition
are the same. Commands that are more interesting will be introduced after
we present our type-level encoding of constraints on states.


==> sections/Introduction.tex <==
%% ODER: format ==         = "\mathrel{==}"
%% ODER: format /=         = "\neq "
%
%
\makeatletter
\@ifundefined{lhs2tex.lhs2tex.sty.read}%
  {\@namedef{lhs2tex.lhs2tex.sty.read}{}%
   \newcommand\SkipToFmtEnd{}%
   \newcommand\EndFmtInput{}%
   \long\def\SkipToFmtEnd#1\EndFmtInput{}%
  }\SkipToFmtEnd

\newcommand\ReadOnlyOnce[1]{\@ifundefined{#1}{\@namedef{#1}{}}\SkipToFmtEnd}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{stmaryrd}
\DeclareFontFamily{OT1}{cmtex}{}
\DeclareFontShape{OT1}{cmtex}{m}{n}
  {<5><6><7><8>cmtex8
   <9>cmtex9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmtex10}{}
\DeclareFontShape{OT1}{cmtex}{m}{it}
  {<-> ssub * cmtt/m/it}{}
\newcommand{\texfamily}{\fontfamily{cmtex}\selectfont}
\DeclareFontShape{OT1}{cmtt}{bx}{n}
  {<5><6><7><8>cmtt8
   <9>cmbtt9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmbtt10}{}
\DeclareFontShape{OT1}{cmtex}{bx}{n}
  {<-> ssub * cmtt/bx/n}{}
\newcommand{\tex}[1]{\text{\texfamily#1}}	% NEU

\newcommand{\Sp}{\hskip.33334em\relax}


\newcommand{\Conid}[1]{\mathit{#1}}
\newcommand{\Varid}[1]{\mathit{#1}}
\newcommand{\anonymous}{\kern0.06em \vbox{\hrule\@width.5em}}
\newcommand{\plus}{\mathbin{+\!\!\!+}}
\newcommand{\bind}{\mathbin{>\!\!\!>\mkern-6.7mu=}}
\newcommand{\rbind}{\mathbin{=\mkern-6.7mu<\!\!\!<}}% suggested by Neil Mitchell
\newcommand{\sequ}{\mathbin{>\!\!\!>}}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\usepackage{polytable}

%mathindent has to be defined
\@ifundefined{mathindent}%
  {\newdimen\mathindent\mathindent\leftmargini}%
  {}%

\def\resethooks{%
  \global\let\SaveRestoreHook\empty
  \global\let\ColumnHook\empty}
\newcommand*{\savecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\savecolumns[#1]}}
\newcommand*{\restorecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\restorecolumns[#1]}}
\newcommand*{\aligncolumn}[2]%
  {\g@addto@macro\ColumnHook{\column{#1}{#2}}}

\resethooks

\newcommand{\onelinecommentchars}{\quad-{}- }
\newcommand{\commentbeginchars}{\enskip\{-}
\newcommand{\commentendchars}{-\}\enskip}

\newcommand{\visiblecomments}{%
  \let\onelinecomment=\onelinecommentchars
  \let\commentbegin=\commentbeginchars
  \let\commentend=\commentendchars}

\newcommand{\invisiblecomments}{%
  \let\onelinecomment=\empty
  \let\commentbegin=\empty
  \let\commentend=\empty}

\visiblecomments

\newlength{\blanklineskip}
\setlength{\blanklineskip}{0.66084ex}

\newcommand{\hsindent}[1]{\quad}% default is fixed indentation
\let\hspre\empty
\let\hspost\empty
\newcommand{\NB}{\textbf{NB}}
\newcommand{\Todo}[1]{$\langle$\textbf{To do:}~#1$\rangle$}

\EndFmtInput
\makeatother
%
%
%
%
%
%
% This package provides two environments suitable to take the place
% of hscode, called "plainhscode" and "arrayhscode". 
%
% The plain environment surrounds each code block by vertical space,
% and it uses \abovedisplayskip and \belowdisplayskip to get spacing
% similar to formulas. Note that if these dimensions are changed,
% the spacing around displayed math formulas changes as well.
% All code is indented using \leftskip.
%
% Changed 19.08.2004 to reflect changes in colorcode. Should work with
% CodeGroup.sty.
%
\ReadOnlyOnce{polycode.fmt}%
\makeatletter

\newcommand{\hsnewpar}[1]%
  {{\parskip=0pt\parindent=0pt\par\vskip #1\noindent}}

% can be used, for instance, to redefine the code size, by setting the
% command to \small or something alike
\newcommand{\hscodestyle}{}

% The command \sethscode can be used to switch the code formatting
% behaviour by mapping the hscode environment in the subst directive
% to a new LaTeX environment.

\newcommand{\sethscode}[1]%
  {\expandafter\let\expandafter\hscode\csname #1\endcsname
   \expandafter\let\expandafter\endhscode\csname end#1\endcsname}

% "compatibility" mode restores the non-polycode.fmt layout.

\newenvironment{compathscode}%
  {\par\noindent
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \let\hspre\(\let\hspost\)%
   \pboxed}%
  {\endpboxed\)%
   \par\noindent
   \ignorespacesafterend}

\newcommand{\compaths}{\sethscode{compathscode}}

% "plain" mode is the proposed default.
% It should now work with \centering.
% This required some changes. The old version
% is still available for reference as oldplainhscode.

\newenvironment{plainhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\hspre\(\let\hspost\)%
   \pboxed}%
  {\endpboxed%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

\newenvironment{oldplainhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

% Here, we make plainhscode the default environment.

\newcommand{\plainhs}{\sethscode{plainhscode}}
\newcommand{\oldplainhs}{\sethscode{oldplainhscode}}
\plainhs

% The arrayhscode is like plain, but makes use of polytable's
% parray environment which disallows page breaks in code blocks.

\newenvironment{arrayhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\parray}%
  {\endparray\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

\newcommand{\arrayhs}{\sethscode{arrayhscode}}

% The mathhscode environment also makes use of polytable's parray 
% environment. It is supposed to be used only inside math mode 
% (I used it to typeset the type rules in my thesis).

\newenvironment{mathhscode}%
  {\parray}{\endparray}

\newcommand{\mathhs}{\sethscode{mathhscode}}

% texths is similar to mathhs, but works in text mode.

\newenvironment{texthscode}%
  {\(\parray}{\endparray\)}

\newcommand{\texths}{\sethscode{texthscode}}

% The framed environment places code in a framed box.

\def\codeframewidth{\arrayrulewidth}
\RequirePackage{calc}

\newenvironment{framedhscode}%
  {\parskip=\abovedisplayskip\par\noindent
   \hscodestyle
   \arrayrulewidth=\codeframewidth
   \tabular{@{}|p{\linewidth-2\arraycolsep-2\arrayrulewidth-2pt}|@{}}%
   \hline\framedhslinecorrect\\{-1.5ex}%
   \let\endoflinesave=\\
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \framedhslinecorrect\endoflinesave{.5ex}\hline
   \endtabular
   \parskip=\belowdisplayskip\par\noindent
   \ignorespacesafterend}

\newcommand{\framedhslinecorrect}[2]%
  {#1[#2]}

\newcommand{\framedhs}{\sethscode{framedhscode}}

% The inlinehscode environment is an experimental environment
% that can be used to typeset displayed code inline.

\newenvironment{inlinehscode}%
  {\(\def\column##1##2{}%
   \let\>\undefined\let\<\undefined\let\\\undefined
   \newcommand\>[1][]{}\newcommand\<[1][]{}\newcommand\\[1][]{}%
   \def\fromto##1##2##3{##3}%
   \def\nextline{}}{\) }%

\newcommand{\inlinehs}{\sethscode{inlinehscode}}

% The joincode environment is a separate environment that
% can be used to surround and thereby connect multiple code
% blocks.

\newenvironment{joincode}%
  {\let\orighscode=\hscode
   \let\origendhscode=\endhscode
   \def\endhscode{\def\hscode{\endgroup\def\@currenvir{hscode}\\}\begingroup}
   %\let\SaveRestoreHook=\empty
   %\let\ColumnHook=\empty
   %\let\resethooks=\empty
   \orighscode\def\hscode{\endgroup\def\@currenvir{hscode}}}%
  {\origendhscode
   \global\let\hscode=\orighscode
   \global\let\endhscode=\origendhscode}%

\makeatother
\EndFmtInput
%

\ReadOnlyOnce{Formatting.fmt}%
\makeatletter

\let\Varid\mathit
\let\Conid\mathsf

\def\commentbegin{\quad\{\ }
\def\commentend{\}}

\newcommand{\ty}[1]{\Conid{#1}}
\newcommand{\con}[1]{\Conid{#1}}
\newcommand{\id}[1]{\Varid{#1}}
\newcommand{\cl}[1]{\Varid{#1}}
\newcommand{\opsym}[1]{\mathrel{#1}}

\newcommand\Keyword[1]{\textbf{\textsf{#1}}}
\newcommand\Hide{\mathbin{\downarrow}}
\newcommand\Reveal{\mathbin{\uparrow}}


%% Paper-specific keywords


\makeatother
\EndFmtInput

\section{Introduction}
\label{sec:introduction}

\Redis{}\footnote{\url{https://redis.io}} is an open source, in-memory data
structure store that can be used as database, cache, and message broker.
A \Redis{} data store can be thought of as a set of key-value pairs. The value
can be a string, a list of strings, a set of strings, or a hash table of
strings, etc. However, string is the only primitive datatype. Numbers, for
example, are serialized to strings before being saved in the data store, and
parsed back to numbers to be manipulated with. While the concept is simple,
\Redis{} is used as an essential component in a number of popular, matured services, including Twitter, GitHub, Weibo, StackOverflow, and Flickr.

For an example, consider the following sequence of commands, entered through the
interactive interface of \Redis{}. The keys \texttt{some-set} and
\texttt{another-set} are both assigned a set of strings. The two calls to
command \texttt{SADD} respectively add three and two strings to the two sets,
before \texttt{SINTER} takes their intersection:
\begin{Verbatim}[xleftmargin=.4in]
redis> SADD some-set a b c
(integer) 3
redis> SADD another-set a b
(integer) 2
redis> SINTER some-set another-set
1) "a"
2) "b"
\end{Verbatim}
\noindent Notice that the keys \texttt{some-set} and \texttt{another-set}, if
not existing before the call to \texttt{SADD}, are created on site. The calls to
\texttt{SADD} return the sizes of the resulting sets.

Many third party libraries provide interfaces for general purpose programming
languages to access \Redis{} through its TCP protocol. For Haskell, the most
popular library is
\Hedis{}.\footnote{\url{https://hackage.haskell.org/package/hedis}}
A (normal) \Redis{} computation returning a value of type \ensuremath{\Varid{a}} is represented in
Haskell by \ensuremath{\Conid{Redis}\;(\Conid{Either}\;\Conid{Reply}\;\Varid{a})}, where the type \ensuremath{\Conid{Redis}} is a monad, while
\ensuremath{\Conid{Either}\;\Conid{Reply}\;\Varid{a}} indicates that the computation either returns a value of type
\ensuremath{\Varid{a}}, or fails with an error message represented by type \ensuremath{\Conid{Reply}}. The following
program implements the previous example:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{15}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{program}\mathbin{::}\Conid{Redis}\;(\Conid{Either}\;\Conid{Reply}\;[\mskip1.5mu \Conid{ByteString}\mskip1.5mu]){}\<[E]%
\\
\>[B]{}\Varid{program}\mathrel{=}\mathbf{do}\;{}\<[15]%
\>[15]{}\Varid{sadd}\;\text{\tt \char34 some-set\char34}\;[\mskip1.5mu \text{\tt \char34 a\char34},\text{\tt \char34 b\char34}\mskip1.5mu]{}\<[E]%
\\
\>[15]{}\Varid{sadd}\;\text{\tt \char34 another-set\char34}\;[\mskip1.5mu \text{\tt \char34 a\char34},\text{\tt \char34 b\char34},\text{\tt \char34 c\char34}\mskip1.5mu]{}\<[E]%
\\
\>[15]{}\Varid{sinter}\;[\mskip1.5mu \text{\tt \char34 some-set\char34},\text{\tt \char34 another-set\char34}\mskip1.5mu]~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
The function
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{10}{@{}>{\hspre}l<{\hspost}@{}}%
\column{12}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{sadd}\mathbin{::}{}\<[10]%
\>[10]{}\Conid{ByteString}\to [\mskip1.5mu \Conid{ByteString}\mskip1.5mu]\to {}\<[E]%
\\
\>[10]{}\hsindent{2}{}\<[12]%
\>[12]{}\Conid{Redis}\;(\Conid{Either}\;\Conid{Reply}\;\Conid{Integer}){}\<[E]%
\ColumnHook
\end{hscode}\resethooks
takes a key and a list of values as arguments, and returns a
\Redis{} computation yielding \ensuremath{\Conid{Integer}}. Keys and values, being nothing but
binary strings in \Redis{}, are represented using Haskell \ensuremath{\Conid{ByteString}}.

\paragraph{The Problems} Most commands work only with data of certain types. In
the following example, the key \texttt{some-string} is assigned a string
\texttt{foo} --- the command \texttt{SET} always assigns a string to a key.
The subsequent call to \texttt{SADD}, which adds a value to a set, thus raises a
runtime error.
\begin{Verbatim}[xleftmargin=.4in]
redis> SET some-string foo
OK
redis> SADD some-string bar
(error) WRONGTYPE Operation against a key
holding the wrong kind of value
\end{Verbatim}
\noindent For another source of type error, the command \texttt{INCR key}
increments the value associated with \texttt{key} by one. With strings being the
only primitive type, \Redis{} parses the stored string to an integer and, after
incrementation, stores a string back. If the string cannot be parsed as an
integer, a runtime error is raised.

We point out a peculiar pattern of value creation and updating
in \Redis{}: the same command is used both to create a key-value pair and to
update them. Similar to \texttt{SADD}, the command \texttt{LPUSH} appends a
value (a string) to a list, or creates one if the key does not exist:
\begin{Verbatim}[xleftmargin=.4in]
redis> LPUSH some-list bar
(integer) 1
\end{Verbatim}
\noindent Another command \texttt{LLEN} returns the length of the list, and
signals an error if the key is not associated with a list:
\begin{Verbatim}[xleftmargin=.4in]
redis> LLEN some-list
(integer) 1
redis> SET some-string foo
OK
redis> LLEN some-string
(error) WRONGTYPE Operation against a key
holding the wrong kind of value
\end{Verbatim}
\noindent Curiously, however, when applied to a key not yet created, \Redis{}
designers chose to let \texttt{LLEN} return \texttt{0}:
\begin{Verbatim}[xleftmargin=.4in]
redis> LLEN nonexistent
(integer) 0
\end{Verbatim}

Being a simple wrapper on top of the TCP protocol of \Redis{}, \Hedis{}
inherits all the behaviors. Executing the following program yields the same
error, but wrapped in a Haskell constructor: \ensuremath{\Conid{Left}\;(\Conid{Error}} \texttt{"WRONGTYPE
Operation against a key holding the wrong kind of value"}\ensuremath{)}.
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{15}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\Varid{program}\mathbin{::}\Conid{Redis}\;(\Conid{Either}\;\Conid{Reply}\;\Conid{Integer}){}\<[E]%
\\
\>[B]{}\Varid{program}\mathrel{=}\mathbf{do}\;{}\<[15]%
\>[15]{}\Varid{set}\;\text{\tt \char34 some-string\char34}\;\text{\tt \char34 foo\char34}{}\<[E]%
\\
\>[15]{}\Varid{sadd}\;\text{\tt \char34 some-string\char34}\;[\mskip1.5mu \text{\tt \char34 a\char34}\mskip1.5mu]~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks

Such a programming model is certainly very error-prone. Working within Haskell,
a host language with a strong typing system, one naturally wishes to build a
domain-specific embedded language (DSEL) that exploits the rich type system
of Haskell to not only ensure the absence of \Redis{} type errors (at least in the simplified situation where there is one client accessing the store), but also
provides better documentations. We wish to be sure that a program calling
\texttt{INCR}, for example, can be type checked only if we can statically
guarantee that the value to be accessed is indeed an integer. We wish to see
from the type of operators such as \texttt{LLEN} when it can be called, and
allow it to be used only in contexts that are safe. We may even want to
explicitly declare a fresh key and its type, to avoid reusing an existing key
by accident, and to prevent it from unexpectedly being used as some other type.

This paper discusses the techniques we used and the experiences we learned from
building such a language, \Edis{}. We constructed an {\em indexed monad}, on
top of the monad \ensuremath{\Conid{Redis}}, which is indexed by a dictionary that maintains the
set of currently defined keys and their types. To represent the dictionary, we
need to encode variable bindings with {\em type-level} lists and strings. And
to manipulate the dictionary, we applied various type-level programming
techniques. To summarize our contributions:
\begin{itemize}
\item We present \Edis{}, a statically typed domain-specific language embedded in Haskell (with extension provided by the Glasgow Haskell Compiler) and built on \Hedis{}. Serializable Haskell datatypes are
automatically converted before being written to \Redis{} data store. Available
keys and their types are kept track of in type-level dictionaries. The types of
embedded commands state clearly their preconditions and postconditions on the
available keys and types, and a program is allowed to be constructed only if
it is guaranteed not to fail with a type error, assuming that it is the only client accessing the store.
%
\item We demonstrate the use of various type-level programming techniques,
including data kinds, singleton types and proxies, closed type families, etc.,
to define type-level lists and operations that observe and manipulate the lists.
%
\item This is (yet another) example of encoding effects and constraints of programs in types, using indexed monad~\cite{indexedmonad}, closed
type-families~\cite{tfclosed} and constraint kinds~\cite{constraintskinds}.
\end{itemize}

In Section~\ref{sec:indexed-monads} we introduce indexed monads, to reason about
pre and postconditions of stateful programs, and in Section~\ref{sec:type-level-dict} we review the basics of type-level
programming in Haskell that allows us to build type-level dictionaries to keep
track of keys and types. Embeddings of \Redis{} commands are presented in
Section~\ref{sec:embedding-commands}. In Section~\ref{sec:discussions} we
discuss various issues regarding design choices, limitations of this approach,
as well as possible future works, before we review related work in
Section~\ref{sec:conclusions}.


==> sections/TypeLevelDict-orig.tex <==
%% ODER: format ==         = "\mathrel{==}"
%% ODER: format /=         = "\neq "
%
%
\makeatletter
\@ifundefined{lhs2tex.lhs2tex.sty.read}%
  {\@namedef{lhs2tex.lhs2tex.sty.read}{}%
   \newcommand\SkipToFmtEnd{}%
   \newcommand\EndFmtInput{}%
   \long\def\SkipToFmtEnd#1\EndFmtInput{}%
  }\SkipToFmtEnd

\newcommand\ReadOnlyOnce[1]{\@ifundefined{#1}{\@namedef{#1}{}}\SkipToFmtEnd}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{stmaryrd}
\DeclareFontFamily{OT1}{cmtex}{}
\DeclareFontShape{OT1}{cmtex}{m}{n}
  {<5><6><7><8>cmtex8
   <9>cmtex9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmtex10}{}
\DeclareFontShape{OT1}{cmtex}{m}{it}
  {<-> ssub * cmtt/m/it}{}
\newcommand{\texfamily}{\fontfamily{cmtex}\selectfont}
\DeclareFontShape{OT1}{cmtt}{bx}{n}
  {<5><6><7><8>cmtt8
   <9>cmbtt9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmbtt10}{}
\DeclareFontShape{OT1}{cmtex}{bx}{n}
  {<-> ssub * cmtt/bx/n}{}
\newcommand{\tex}[1]{\text{\texfamily#1}}	% NEU

\newcommand{\Sp}{\hskip.33334em\relax}


\newcommand{\Conid}[1]{\mathit{#1}}
\newcommand{\Varid}[1]{\mathit{#1}}
\newcommand{\anonymous}{\kern0.06em \vbox{\hrule\@width.5em}}
\newcommand{\plus}{\mathbin{+\!\!\!+}}
\newcommand{\bind}{\mathbin{>\!\!\!>\mkern-6.7mu=}}
\newcommand{\rbind}{\mathbin{=\mkern-6.7mu<\!\!\!<}}% suggested by Neil Mitchell
\newcommand{\sequ}{\mathbin{>\!\!\!>}}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\usepackage{polytable}

%mathindent has to be defined
\@ifundefined{mathindent}%
  {\newdimen\mathindent\mathindent\leftmargini}%
  {}%

\def\resethooks{%
  \global\let\SaveRestoreHook\empty
  \global\let\ColumnHook\empty}
\newcommand*{\savecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\savecolumns[#1]}}
\newcommand*{\restorecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\restorecolumns[#1]}}
\newcommand*{\aligncolumn}[2]%
  {\g@addto@macro\ColumnHook{\column{#1}{#2}}}

\resethooks

\newcommand{\onelinecommentchars}{\quad-{}- }
\newcommand{\commentbeginchars}{\enskip\{-}
\newcommand{\commentendchars}{-\}\enskip}

\newcommand{\visiblecomments}{%
  \let\onelinecomment=\onelinecommentchars
  \let\commentbegin=\commentbeginchars
  \let\commentend=\commentendchars}

\newcommand{\invisiblecomments}{%
  \let\onelinecomment=\empty
  \let\commentbegin=\empty
  \let\commentend=\empty}

\visiblecomments

\newlength{\blanklineskip}
\setlength{\blanklineskip}{0.66084ex}

\newcommand{\hsindent}[1]{\quad}% default is fixed indentation
\let\hspre\empty
\let\hspost\empty
\newcommand{\NB}{\textbf{NB}}
\newcommand{\Todo}[1]{$\langle$\textbf{To do:}~#1$\rangle$}

\EndFmtInput
\makeatother
%
%
%
%
%
%
% This package provides two environments suitable to take the place
% of hscode, called "plainhscode" and "arrayhscode". 
%
% The plain environment surrounds each code block by vertical space,
% and it uses \abovedisplayskip and \belowdisplayskip to get spacing
% similar to formulas. Note that if these dimensions are changed,
% the spacing around displayed math formulas changes as well.
% All code is indented using \leftskip.
%
% Changed 19.08.2004 to reflect changes in colorcode. Should work with
% CodeGroup.sty.
%
\ReadOnlyOnce{polycode.fmt}%
\makeatletter

\newcommand{\hsnewpar}[1]%
  {{\parskip=0pt\parindent=0pt\par\vskip #1\noindent}}

% can be used, for instance, to redefine the code size, by setting the
% command to \small or something alike
\newcommand{\hscodestyle}{}

% The command \sethscode can be used to switch the code formatting
% behaviour by mapping the hscode environment in the subst directive
% to a new LaTeX environment.

\newcommand{\sethscode}[1]%
  {\expandafter\let\expandafter\hscode\csname #1\endcsname
   \expandafter\let\expandafter\endhscode\csname end#1\endcsname}

% "compatibility" mode restores the non-polycode.fmt layout.

\newenvironment{compathscode}%
  {\par\noindent
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \let\hspre\(\let\hspost\)%
   \pboxed}%
  {\endpboxed\)%
   \par\noindent
   \ignorespacesafterend}

\newcommand{\compaths}{\sethscode{compathscode}}

% "plain" mode is the proposed default.
% It should now work with \centering.
% This required some changes. The old version
% is still available for reference as oldplainhscode.

\newenvironment{plainhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\hspre\(\let\hspost\)%
   \pboxed}%
  {\endpboxed%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

\newenvironment{oldplainhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

% Here, we make plainhscode the default environment.

\newcommand{\plainhs}{\sethscode{plainhscode}}
\newcommand{\oldplainhs}{\sethscode{oldplainhscode}}
\plainhs

% The arrayhscode is like plain, but makes use of polytable's
% parray environment which disallows page breaks in code blocks.

\newenvironment{arrayhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\parray}%
  {\endparray\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

\newcommand{\arrayhs}{\sethscode{arrayhscode}}

% The mathhscode environment also makes use of polytable's parray 
% environment. It is supposed to be used only inside math mode 
% (I used it to typeset the type rules in my thesis).

\newenvironment{mathhscode}%
  {\parray}{\endparray}

\newcommand{\mathhs}{\sethscode{mathhscode}}

% texths is similar to mathhs, but works in text mode.

\newenvironment{texthscode}%
  {\(\parray}{\endparray\)}

\newcommand{\texths}{\sethscode{texthscode}}

% The framed environment places code in a framed box.

\def\codeframewidth{\arrayrulewidth}
\RequirePackage{calc}

\newenvironment{framedhscode}%
  {\parskip=\abovedisplayskip\par\noindent
   \hscodestyle
   \arrayrulewidth=\codeframewidth
   \tabular{@{}|p{\linewidth-2\arraycolsep-2\arrayrulewidth-2pt}|@{}}%
   \hline\framedhslinecorrect\\{-1.5ex}%
   \let\endoflinesave=\\
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \framedhslinecorrect\endoflinesave{.5ex}\hline
   \endtabular
   \parskip=\belowdisplayskip\par\noindent
   \ignorespacesafterend}

\newcommand{\framedhslinecorrect}[2]%
  {#1[#2]}

\newcommand{\framedhs}{\sethscode{framedhscode}}

% The inlinehscode environment is an experimental environment
% that can be used to typeset displayed code inline.

\newenvironment{inlinehscode}%
  {\(\def\column##1##2{}%
   \let\>\undefined\let\<\undefined\let\\\undefined
   \newcommand\>[1][]{}\newcommand\<[1][]{}\newcommand\\[1][]{}%
   \def\fromto##1##2##3{##3}%
   \def\nextline{}}{\) }%

\newcommand{\inlinehs}{\sethscode{inlinehscode}}

% The joincode environment is a separate environment that
% can be used to surround and thereby connect multiple code
% blocks.

\newenvironment{joincode}%
  {\let\orighscode=\hscode
   \let\origendhscode=\endhscode
   \def\endhscode{\def\hscode{\endgroup\def\@currenvir{hscode}\\}\begingroup}
   %\let\SaveRestoreHook=\empty
   %\let\ColumnHook=\empty
   %\let\resethooks=\empty
   \orighscode\def\hscode{\endgroup\def\@currenvir{hscode}}}%
  {\origendhscode
   \global\let\hscode=\orighscode
   \global\let\endhscode=\origendhscode}%

\makeatother
\EndFmtInput
%

\ReadOnlyOnce{Formatting.fmt}%
\makeatletter

\let\Varid\mathit
\let\Conid\mathsf

\def\commentbegin{\quad\{\ }
\def\commentend{\}}

\newcommand{\ty}[1]{\Conid{#1}}
\newcommand{\con}[1]{\Conid{#1}}
\newcommand{\id}[1]{\Varid{#1}}
\newcommand{\cl}[1]{\Varid{#1}}
\newcommand{\opsym}[1]{\mathrel{#1}}

\newcommand\Keyword[1]{\textbf{\textsf{#1}}}
\newcommand\Hide{\mathbin{\downarrow}}
\newcommand\Reveal{\mathbin{\uparrow}}


%% Paper-specific keywords


\makeatother
\EndFmtInput

\section{Type-Level Dictionaries}
\label{sec:type-level-dict}

One of the challenges of statically ensuring type correctness of stateful
languages is that the type of the value of a key can be altered by updating.
In \Redis{}, one may delete an existing key and create it again by assigning to
it a value of a different type. To ensure type correctness, we keep track of the
types of all existing keys in a {\em dictionary} --- an associate list, or a
list of pairs of keys and some encoding of types. For example, we may use the
dictionary \ensuremath{[\mskip1.5mu (\text{\tt \char34 A\char34},\Conid{Int}),(\text{\tt \char34 B\char34},\Conid{Char}),(\text{\tt \char34 C\char34},\Conid{Bool})\mskip1.5mu]} to represent a
predicate, or a constraint, stating that ``the keys in the data store are \ensuremath{\text{\tt \char34 A\char34}},
\ensuremath{\text{\tt \char34 B\char34}}, and \ensuremath{\text{\tt \char34 C\char34}}, respectively assigned values of type \ensuremath{\Conid{Int}}, \ensuremath{\Conid{Char}}, and
\ensuremath{\Conid{Bool}}.'' (This representation will be refined in the next section.)

The dictionary above mixes values (strings such as \ensuremath{\text{\tt \char34 A\char34}}, \ensuremath{\text{\tt \char34 B\char34}}) and types.
Furthermore, as mentioned in Section~\ref{sec:indexed-monads}, the
dictionaries will be parameters to the indexed monad \ensuremath{\Conid{Edis}}. In a dependently
typed programming language (without the so-called ``phase distinction'' ---
separation between types and terms), this would pose no problem. In Haskell
however, the dictionaries, to index a monad, has to be a type as well.

In this section we describe how to construct a type-level dictionary, to be
used with the indexed monad in Section~\ref{sec:indexed-monads}.

\subsection{Datatype Promotion}

Haskell maintains the distinction between values, types, and kinds: values are
categorized by types, and types are categorized by kinds. The kinds are
relatively simple: \ensuremath{\mathbin{*}} is the kind of all {\em lifted} types, while type
constructors have kinds such as \ensuremath{\mathbin{*}\to \mathbin{*}}, or \ensuremath{\mathbin{*}\to \mathbin{*}\to \mathbin{*}}, etc.\footnotemark\,
Consider the datatype definitions below:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\mathbf{data}\;\Conid{Nat}\mathrel{=}\Conid{Zero}\mid \Conid{Suc}\;\Conid{Nat}~~,\qquad\;\mathbf{data}\;[\mskip1.5mu \Varid{a}\mskip1.5mu]\mathrel{=}[\mskip1.5mu \mskip1.5mu]\mid \Varid{a}\mathbin{:}[\mskip1.5mu \Varid{a}\mskip1.5mu]~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
The left-hand side is usually seen as having defined a type \ensuremath{\Conid{Nat}\mathbin{::}\mathbin{*}},
and two value constructors \ensuremath{\Conid{Zero}\mathbin{::}\Conid{Nat}} and \ensuremath{\Conid{Suc}\mathbin{::}\Conid{Nat}\to \Conid{Nat}}. The right-hand
side is how Haskell lists are understood. The {\em kind} of \ensuremath{[\mskip1.5mu \mathbin{\cdot}\mskip1.5mu]} is \ensuremath{\mathbin{*}\to \mathbin{*}},
since it takes a lifted type \ensuremath{\Varid{a}} to a lifted type \ensuremath{[\mskip1.5mu \Varid{a}\mskip1.5mu]}. The two value
constructors respectively have types \ensuremath{[\mskip1.5mu \mskip1.5mu]\mathbin{::}[\mskip1.5mu \Varid{a}\mskip1.5mu]} and \ensuremath{(\mathbin{:})\mathbin{::}\Varid{a}\to [\mskip1.5mu \Varid{a}\mskip1.5mu]\to [\mskip1.5mu \Varid{a}\mskip1.5mu]}, for all type \ensuremath{\Varid{a}}.

\footnotetext{In Haskell, the opposite of \emph{lifted} types are \emph{unboxed}
types, which are not represented by a pointer to a heap object, and cannot be
stored in a polymorphic data type.}

The GHC extension \emph{data kinds}~\cite{promotion}, however, automatically
promotes certain ``suitable'' types to kinds.\footnote{It is only informally
described in the GHC manual what types are ``suitable''.} With the extension,
the \ensuremath{\mathbf{data}} definitions above has an alternative reading: \ensuremath{\Conid{Nat}} is a new kind,
\ensuremath{\Conid{Zero}\mathbin{::}\Conid{Nat}} is a type having kind \ensuremath{\Conid{Nat}}, and \ensuremath{\Conid{Suc}\mathbin{::}\Conid{Nat}\to \Conid{Nat}} is a type
constructor, taking a type in kind \ensuremath{\Conid{Nat}} to another type in \ensuremath{\Conid{Nat}}. When one
sees a constructor in an expression, whether it is promoted can often be
inferred from the context. When one needs to be more specific, prefixing a
constructor with a single quote, such as in \ensuremath{\mbox{\textquotesingle}\Conid{Zero}} and \ensuremath{\mbox{\textquotesingle}\Conid{Suc}}, denotes that it
is promoted.

The situation of lists is similar: for all kind \ensuremath{\Varid{k}}, \ensuremath{[\mskip1.5mu \Varid{k}\mskip1.5mu]} is also a kind. For
all kind \ensuremath{\Varid{k}}, \ensuremath{[\mskip1.5mu \mskip1.5mu]} is a type of kind \ensuremath{[\mskip1.5mu \Varid{k}\mskip1.5mu]}. Given a type \ensuremath{\Varid{a}} of kind \ensuremath{\Varid{k}} and a
type \ensuremath{\Varid{as}} of kind \ensuremath{[\mskip1.5mu \Varid{k}\mskip1.5mu]}, \ensuremath{\Varid{a}\mathbin{:}\Varid{as}} is again a type of kind \ensuremath{[\mskip1.5mu \Varid{k}\mskip1.5mu]}. Formally,
\ensuremath{(\mathbin{:})\mathbin{::}\Varid{k}\to [\mskip1.5mu \Varid{k}\mskip1.5mu]\to [\mskip1.5mu \Varid{k}\mskip1.5mu]}. For example, \ensuremath{\Conid{Int}\mathrel{\,\mbox{\textquotesingle}\!:}(\Conid{Char}\mathrel{\,\mbox{\textquotesingle}\!:}(\Conid{Bool}\mathrel{\,\mbox{\textquotesingle}\!:}\mbox{\textquotesingle}[~]))} is a
type having kind \ensuremath{[\mskip1.5mu \mathbin{*}\mskip1.5mu]} --- it is a list of (lifted) types. The optional quote
denotes that the constructors are promoted. The same list can be denoted by a
syntax sugar \ensuremath{\mbox{\textquotesingle}[\Conid{Int},\Conid{Char},\Conid{Bool}]}.

Tuples are also promoted. Thus we may put two types in a pair to form another
type, such as in \ensuremath{\mbox{\textquotesingle}(\Conid{Int},\Conid{Char})}, a type having kind \ensuremath{(\mathbin{*},\mathbin{*})}.

Strings in Haskell are nothing but lists of \ensuremath{\Conid{Char}}s. Regarding promotion,
however, a string can be promoted to a type having kind \ensuremath{\Conid{Symbol}}. In the expression:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\text{\tt \char34 this~is~a~type-level~string~literal\char34}\mathbin{::}\Conid{Symbol}~~,{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
the string on the left-hand side of \ensuremath{(\mathbin{::})} is a type whose kind is \ensuremath{\Conid{Symbol}}.

With all of these ingredients, we are ready to build our dictionaries, or
type-level associate lists:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\mathbf{type}\;\Conid{DictEmpty}\mathrel{=}\mbox{\textquotesingle}[~]~~,{}\<[E]%
\\
\>[B]{}\mathbf{type}\;\Conid{Dict0}\mathrel{=}\mbox{\textquotesingle}[\mbox{\textquotesingle}(\text{\tt \char34 key\char34},\Conid{Bool})]~~,{}\<[E]%
\\
\>[B]{}\mathbf{type}\;\Conid{Dict1}\mathrel{=}\mbox{\textquotesingle}[\mbox{\textquotesingle}(\text{\tt \char34 A\char34},\Conid{Int}),\mbox{\textquotesingle}(\text{\tt \char34 B\char34},\text{\tt \char34 A\char34})]~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
All the entities defined above are types, where \ensuremath{\Conid{Dict0}} has kind \ensuremath{[\mskip1.5mu (\Conid{Symbol},\mathbin{*})\mskip1.5mu]}. In \ensuremath{\Conid{Dict1}}, while \ensuremath{\Conid{Int}} has kind \ensuremath{\mathbin{*}} and \ensuremath{\text{\tt \char34 A\char34}} has kind \ensuremath{\Conid{Symbol}}, the former kind subsumes the later. Thus \ensuremath{\Conid{Dict1}} also has kind \ensuremath{[\mskip1.5mu (\Conid{Symbol},\mathbin{*})\mskip1.5mu]}.

\subsection{Type-Level Functions}
\label{sec:type-fun}

Now that we can represent dictionaries as types, the next step is to define
operations on them. A function that inserts an entry to a dictionary, for
example, is a function from a type to a type. While it was shown that it is
possible to simulate type-level functions using Haskell type
classes~\cite{McBride:02:Faking}, in recent versions of GHC, {\em indexed type
families}, or \emph{type families} for short, are considered a cleaner solution.

For example, compare disjunction \ensuremath{(\mathrel{\vee})} and its type-level
counterpart:\\
\noindent{\centering %\small
\begin{minipage}[b]{0.35\linewidth}
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{7}{@{}>{\hspre}c<{\hspost}@{}}%
\column{7E}{@{}l@{}}%
\column{11}{@{}>{\hspre}l<{\hspost}@{}}%
\column{14}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}(\mathrel{\vee})\mathbin{::}\Conid{Bool}\to \Conid{Bool}\to \Conid{Bool}{}\<[E]%
\\
\>[B]{}\Conid{True}{}\<[7]%
\>[7]{}\mathrel{\vee}{}\<[7E]%
\>[11]{}\Varid{b}{}\<[14]%
\>[14]{}\mathrel{=}\Conid{True}{}\<[E]%
\\
\>[B]{}\Varid{a}{}\<[7]%
\>[7]{}\mathrel{\vee}{}\<[7E]%
\>[11]{}\Varid{b}{}\<[14]%
\>[14]{}\mathrel{=}\Varid{b}~~,{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
\end{minipage}
\begin{minipage}[b]{0.55\linewidth}
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{3}{@{}>{\hspre}l<{\hspost}@{}}%
\column{10}{@{}>{\hspre}l<{\hspost}@{}}%
\column{16}{@{}>{\hspre}l<{\hspost}@{}}%
\column{24}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\mathbf{type}\;\Varid{family}\;\Conid{Or}\;(\Varid{a}\mathbin{::}\Conid{Bool})\;(\Varid{b}\mathbin{::}\Conid{Bool})\mathbin{::}\Conid{Bool}{}\<[E]%
\\
\>[B]{}\hsindent{3}{}\<[3]%
\>[3]{}\mathbf{where}\;{}\<[10]%
\>[10]{}\mbox{\textquotesingle}\Conid{True}{}\<[16]%
\>[16]{}\mathrel{\Conid{`Or`}}\Varid{b}{}\<[24]%
\>[24]{}\mathrel{=}\mbox{\textquotesingle}\Conid{True}{}\<[E]%
\\
\>[10]{}\Varid{a}{}\<[16]%
\>[16]{}\mathrel{\Conid{`Or`}}\Varid{b}{}\<[24]%
\>[24]{}\mathrel{=}\Varid{b}~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
\end{minipage}
}\\
The left-hand side is a typical definition of \ensuremath{(\mathrel{\vee})} by pattern matching.
On the right-hand side, \ensuremath{\Conid{Bool}} is not a type, but a type lifted to a kind,
while \ensuremath{\Conid{True}} and \ensuremath{\Conid{False}} are types of kind \ensuremath{\Conid{Bool}}. The declaration says that
\ensuremath{\Conid{Or}} is a family of types, indexed by two parameters \ensuremath{\Varid{a}} and \ensuremath{\Varid{b}} of kind \ensuremath{\Conid{Bool}}.
The type with index \ensuremath{\mbox{\textquotesingle}\Conid{True}} and \ensuremath{\Varid{b}} is \ensuremath{\mbox{\textquotesingle}\Conid{True}}, and all other indices lead to \ensuremath{\Varid{b}}.
For our purpose, we can read \ensuremath{\Conid{Or}} as a function from types to types ---
observe how it resembles the term-level \ensuremath{(\mathrel{\vee})}. We present two more type-level
functions about \ensuremath{\Conid{Bool}} --- negation, and conditional, that we will use later:\\
\noindent{\centering %\small
\begin{minipage}[b]{0.35\linewidth}
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{3}{@{}>{\hspre}l<{\hspost}@{}}%
\column{14}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\mathbf{type}\;\Varid{family}\;\Conid{Not}\;\Varid{a}\;\mathbf{where}{}\<[E]%
\\
\>[B]{}\hsindent{3}{}\<[3]%
\>[3]{}\Conid{Not}\;\mbox{\textquotesingle}\Conid{False}{}\<[14]%
\>[14]{}\mathrel{=}\mbox{\textquotesingle}\Conid{True}{}\<[E]%
\\
\>[B]{}\hsindent{3}{}\<[3]%
\>[3]{}\Conid{Not}\;\mbox{\textquotesingle}\Conid{True}{}\<[14]%
\>[14]{}\mathrel{=}\mbox{\textquotesingle}\Conid{False}~~,{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
\end{minipage}
\begin{minipage}[b]{0.55\linewidth}
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{3}{@{}>{\hspre}l<{\hspost}@{}}%
\column{12}{@{}>{\hspre}l<{\hspost}@{}}%
\column{17}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\mathbf{type}\;\Varid{family}\;\Conid{If}\;(\Varid{c}\mathbin{::}\Conid{Bool})\;(\Varid{t}\mathbin{::}\Varid{a})\;(\Varid{f}\mathbin{::}\Varid{a})\mathbin{::}\Varid{a}\;\mathbf{where}{}\<[E]%
\\
\>[B]{}\hsindent{3}{}\<[3]%
\>[3]{}\Conid{If}\;\mbox{\textquotesingle}\Conid{True}\;{}\<[12]%
\>[12]{}\Varid{tru}\;{}\<[17]%
\>[17]{}\Varid{fls}\mathrel{=}\Varid{tru}{}\<[E]%
\\
\>[B]{}\hsindent{3}{}\<[3]%
\>[3]{}\Conid{If}\;\mbox{\textquotesingle}\Conid{False}\;\Varid{tru}\;{}\<[17]%
\>[17]{}\Varid{fls}\mathrel{=}\Varid{fls}~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
\end{minipage}
}

As a remark, type families in Haskell come in many flavors. One can define families of \ensuremath{\mathbf{data}}, as well as families of \ensuremath{\mathbf{type}} synonym. They can appear
inside type classes~\cite{tfclass,tfsynonym} or at toplevel. Top-level type families can be open~\cite{tfopen} or closed~\cite{tfclosed}. The flavor we
chose is top-level, closed type synonym family, since it allows overlapping
instances, and since we need none of the extensibility provided by open type
families. Notice that the instance \ensuremath{\mbox{\textquotesingle}\Conid{True}\mathrel{\Conid{`Or`}}\Varid{b}} could be subsumed under the
more general instance, \ensuremath{\Varid{a}\mathrel{\Conid{`Or`}}\Varid{b}}. In a closed type family we may resolve the
overlapping in order, just like how cases overlapping is resolved in term-level
functions.

Now we can define operations on type-level dictionaries. Let us begin
with:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{5}{@{}>{\hspre}l<{\hspost}@{}}%
\column{20}{@{}>{\hspre}l<{\hspost}@{}}%
\column{33}{@{}>{\hspre}c<{\hspost}@{}}%
\column{33E}{@{}l@{}}%
\column{36}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\mathbf{type}\;\Varid{family}\;\Conid{Get}\;(\Varid{xs}\mathbin{::}[\mskip1.5mu (\Conid{Symbol},\mathbin{*})\mskip1.5mu])\;(\Varid{k}\mathbin{::}\Conid{Symbol})\mathbin{::}\mathbin{*}\mathbf{where}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{Get}\;(\mbox{\textquotesingle}(\Varid{k},{}\<[20]%
\>[20]{}\Varid{x})\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;\Varid{k}{}\<[33]%
\>[33]{}\mathrel{=}{}\<[33E]%
\>[36]{}\Varid{x}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{Get}\;(\mbox{\textquotesingle}(\Varid{t},{}\<[20]%
\>[20]{}\Varid{x})\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;\Varid{k}{}\<[33]%
\>[33]{}\mathrel{=}{}\<[33E]%
\>[36]{}\Conid{Get}\;\Varid{xs}\;\Varid{k}~~.{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
\ensuremath{\Conid{Get}\;\Varid{xs}\;\Varid{k}} returns the entry associated with key \ensuremath{\Varid{k}} in the
dictionary \ensuremath{\Varid{xs}}. Notice, in the first case, how type-level equality can be
expressed by unifying type variables with the same name. Note also that \ensuremath{\Conid{Get}} is
a partial function on types: while \ensuremath{\Conid{Get}\;\mbox{\textquotesingle}[\mbox{\textquotesingle}(\text{\tt \char34 A\char34},\Conid{Int})]\;\text{\tt \char34 A\char34}} evaluates
to \ensuremath{\Conid{Int}}, when \ensuremath{\Conid{Get}\;\mbox{\textquotesingle}[\mbox{\textquotesingle}(\text{\tt \char34 A\char34},\Conid{Int})]\;\text{\tt \char34 B\char34}} appears in a type expression,
there are no applicable rules to reduce it. The expression thus stays un-reduced.

% For our applications it is more convenient to make |Get| total, as we would at
% the term level, by having it return a |Maybe|:
% \begin{spec}
% type family Get (xs :: [(Symbol, *)]) (k :: Symbol) :: Maybe * where
%     Get NIL                 k = Nothing
%     Get (TPar(k, x) :- xs)  k = Just x
%     Get (TPar(t, x) :- xs)  k = Get xs k {-"~~."-}
% \end{spec}
%
Some other dictionary-related functions are defined
in Figure \ref{fig:dict-operations}. The function \ensuremath{\Conid{Set}} either updates an
existing entry or inserts a new entry, \ensuremath{\Conid{Del}} removes an entry matching
a given key, while \ensuremath{\Conid{Member}} checks whether a given key exists in the
dictionary.

\begin{figure}[t]
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{5}{@{}>{\hspre}l<{\hspost}@{}}%
\column{18}{@{}>{\hspre}l<{\hspost}@{}}%
\column{29}{@{}>{\hspre}l<{\hspost}@{}}%
\column{30}{@{}>{\hspre}l<{\hspost}@{}}%
\column{33}{@{}>{\hspre}l<{\hspost}@{}}%
\column{48}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[B]{}\mbox{\onelinecomment  inserts or updates an entry}{}\<[E]%
\\
\>[B]{}\mathbf{type}\;\Varid{family}\;\Conid{Set}\;{}\<[18]%
\>[18]{}(\Varid{xs}\mathbin{::}[\mskip1.5mu (\Conid{Symbol},\mathbin{*})\mskip1.5mu])\;(\Varid{k}\mathbin{::}\Conid{Symbol})\;(\Varid{x}\mathbin{::}\mathbin{*})\mathbin{::}[\mskip1.5mu (\Conid{Symbol},\mathbin{*})\mskip1.5mu]\;\mathbf{where}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{Set}\;\mbox{\textquotesingle}[~]\;{}\<[29]%
\>[29]{}\Varid{k}\;\Varid{x}\mathrel{=}\mbox{\textquotesingle}[\mbox{\textquotesingle}(\Varid{k},\Varid{x})]{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{Set}\;(\mbox{\textquotesingle}(\Varid{k},\Varid{y})\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;{}\<[29]%
\>[29]{}\Varid{k}\;\Varid{x}\mathrel{=}\mbox{\textquotesingle}(\Varid{k},\Varid{x}){}\<[48]%
\>[48]{}\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{Set}\;(\mbox{\textquotesingle}(\Varid{t},\Varid{y})\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;{}\<[29]%
\>[29]{}\Varid{k}\;\Varid{x}\mathrel{=}\mbox{\textquotesingle}(\Varid{t},\Varid{y}){}\<[48]%
\>[48]{}\mathrel{\,\mbox{\textquotesingle}\!:}\Conid{Set}\;\Varid{xs}\;\Varid{k}\;\Varid{x}{}\<[E]%
\\[\blanklineskip]%
\>[B]{}\mbox{\onelinecomment  removes an entry}{}\<[E]%
\\
\>[B]{}\mathbf{type}\;\Varid{family}\;\Conid{Del}\;{}\<[18]%
\>[18]{}(\Varid{xs}\mathbin{::}[\mskip1.5mu (\Conid{Symbol},\mathbin{*})\mskip1.5mu])\;(\Varid{k}\mathbin{::}\Conid{Symbol})\mathbin{::}[\mskip1.5mu (\Conid{Symbol},\mathbin{*})\mskip1.5mu]\;\mathbf{where}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{Del}\;\Conid{Nil}\;{}\<[30]%
\>[30]{}\Varid{k}\mathrel{=}\Conid{Nil}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{Del}\;(\mbox{\textquotesingle}(\Varid{k},\Varid{y})\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;{}\<[30]%
\>[30]{}\Varid{k}\mathrel{=}\Varid{xs}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{Del}\;(\mbox{\textquotesingle}(\Varid{t},\Varid{y})\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;{}\<[30]%
\>[30]{}\Varid{k}\mathrel{=}\mbox{\textquotesingle}(\Varid{t},\Varid{y})\mathrel{\,\mbox{\textquotesingle}\!:}\Conid{Del}\;\Varid{xs}\;\Varid{k}{}\<[E]%
\\[\blanklineskip]%
\>[B]{}\mbox{\onelinecomment  membership}{}\<[E]%
\\
\>[B]{}\mathbf{type}\;\Varid{family}\;\Conid{Member}\;(\Varid{xs}\mathbin{::}[\mskip1.5mu (\Conid{Symbol},\mathbin{*})\mskip1.5mu])\;(\Varid{k}\mathbin{::}\Conid{Symbol})\mathbin{::}\Conid{Bool}\;\mathbf{where}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{Member}\;\Conid{Nil}\;{}\<[33]%
\>[33]{}\Varid{k}\mathrel{=}\Conid{False}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{Member}\;(\mbox{\textquotesingle}(\Varid{k},\Varid{x})\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;{}\<[33]%
\>[33]{}\Varid{k}\mathrel{=}\Conid{True}{}\<[E]%
\\
\>[B]{}\hsindent{5}{}\<[5]%
\>[5]{}\Conid{Member}\;(\mbox{\textquotesingle}(\Varid{t},\Varid{x})\mathrel{\,\mbox{\textquotesingle}\!:}\Varid{xs})\;{}\<[33]%
\>[33]{}\Varid{k}\mathrel{=}\Conid{Member}\;\Varid{xs}\;\Varid{k}{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
\caption{Some operations on type-level dictionaries.}
\label{fig:dict-operations}
\end{figure}

